Domain Walls in Supersymmetric Yang-Mills Theories

We study BPS saturated domain walls in the supersymmetric SU(2) gauge theory. For a theory with a very light adjoint scalar (mass <~ Lambda/400) we use the perturbed N=2 Seiberg-Witten theory to calculate the actual field configuration of the domain wall. The wall has a sandwich-like five-layer structure of three distinct phases -- electric confinement, Coulomb and oblique confinement -- separated by two separate transition regions. For larger scalar masses, the three-phase structure disappears and the Seiberg-Witten theory becomes inadequate because of two major problems: First, the higher-derivative interactions between the light fields become relevant and second, both the magnetic monopole condensate and the dyon condensate show up in the same region of space, a phenomenon indescribable in terms of a local field theory. Nevertheless, we argue that the BPS saturated domain wall continues to exist in this regime and give a qualitative description of the scalar and gaugino condensates. Finally, we discuss the domain walls in MQCD and translate the BPS conditions into coupled non-linear differential equations.

==> Appendices.tex <==
%auto-ignore
%
% Appendices to the DomainWall paper
%
\APPENDIX{A}{A\break Higher--Derivative Interactions\break
and their Effect on Auxiliary Fields}

In order to solve eqs.~\val\BPSGeneric\ for a BPS-saturated domain wall
of a $\NS=1$ supersymmetric effective field theory
we need to solve for the auxiliary fields $F^i$ in terms of the
physical scalar fields $A^i$.
In the context of an effective Lagrangian --- or rather the generating
functional $\Gamma$ which we assume to be local, --- the only
terms that remain relevant in the long-distance or low-energy limit
are those with at most four superderivatives,
$$
{\cal L}_{4\nabla}\
=\ -\int\!\!d^4\theta\,K(\overline\Phi,\Phi)\
+ \int\!\!d^2\theta\,\bigl[W(\Phi)+\coeff{\tau(\Phi)}{16\pi i}\,
	W^\alpha W_\alpha\bigr]\
+\ \rm H.\,c.
\eqn\RelevantLagr
$$
Expanding this effective Lagrangian in component fields,
we focus on terms containing the auxiliary fields $F^i$ and
disregard the fermionic fields as not germane to the domain wall.
Thus,
$$
{\cal L}_{4\nabla}\ =\ -g_{i\bar\jmath}\,F^i F^{*\bar\jmath}\
+\ W_i\,F^i\ +\ W^*_{\bar\imath}\,F^{*\bar\imath}\ +\ \cdots
\eqn\Fterms
$$
and hence 
$$
F^i\ =\ g^{i\bar\jmath}W^*_{\bar\jmath}\,.
\eqn\Obvious
$$

Unfortunately, eqs.~\Obvious\ is valid only in the
long-distance limit where ${\cal L}\approx{\cal L}_{4\nabla}$.
At shorter distances or higher energies, the higher-derivative
interaction terms in the effective Lagrangian become relevant too.
At the six superderivative level, we have
$$
\eqalign{
\!{\cal L}_{6\nabla}\ &
=\int\!\!d^4\theta\,\Bigl[
    L_{ij}(\overline\Phi,\Phi)\,\nabla^\alpha\Phi^i\nabla_\alpha\Phi^j\
    +\ H(\overline\Phi,\Phi)\,W^\alpha W_\alpha\ +\ \rm H.\,c.\,\Bigr]\cr
&=\ L_{ij}\,F^i \nabla^\mu \nabla_\mu A^j\
    +\ L_{(ij,k)}\,F^i \nabla^\mu A^j \nabla_\mu A^k\cr
&\quad+\ L_{ij,\bar k}\,F^i F^j F^{*\bar k}\
    +\ H_{\bar\imath}\,F^{*\bar\imath}
	\left( D^2+\coeff14 (F_{\mu\nu}+\tilde F_{\mu\nu})^2\right)\cr
&\quad+\ \rm H.\,c.\ +\ \cdots\cr
}\eqn\SixDerivatives
$$
where the `$\cdots$' again stands for the fermionic terms or terms
not involving the auxiliary fields $F^i$ and $F^{*\bar\jmath}$.
The effect of the the six-super\-derivative interactions \SixDerivatives\
on the field equations for the auxiliary fields
is to replace eqs.~\Obvious\ with  messy, non-linear equations:
$$
\eqalign{
g_{\bar\imath j}F^j\ =\ W^*_{\bar\imath}\ &
+\ L_{jk,\bar\imath}\,F^j F^k\
    +\ 2L^*_{\bar\imath\bar\jmath,k}\,F^{*\bar\jmath} F^k\
    +\ L^*_{(\bar\imath\bar\jmath,\bar k)}\,
	\nabla^\mu A^{*\bar\jmath}\, \nabla_\mu A^{*\bar k}\cr
&+\ L^*_{\bar\imath\bar\jmath}\,\nabla^\mu\nabla_\mu A^{*\bar\jmath}\
    +\ H_{\bar\imath}\left( D^2+\coeff14 (F_{\mu\nu}+\tilde F_{\mu\nu})^2\right).
}\eqn\DVIFeq
$$

At the eight superderivative level (and beyond), the field equations
for the $F^i$ fields become not just non-linear but differential
rather than algebraic.
As an example of an eight-super\-derivative terms, consider
$$
\int\!\!d^4\theta\,\coeff{1}{16} N_{\bar\imath j}(\overline\Phi,\Phi)\,
	\nabla^{\dot\alpha}\nabla_{\dot\alpha}
		\smash{\overline\Phi}\vphantom{\Phi}^{\bar\imath}\,
	\nabla^\alpha\nabla_\alpha \Phi^j
\eqn\EightDerivatives
$$
which expands to
$$
\eqalign{
N_{\bar\imath j}\,\nabla^\mu F^{*\bar\imath}\,\nabla_\mu F^j\ &
+\ N_{\bar\imath j,k\bar\ell}\,F^{*\bar\imath}F^j\left(
	\nabla^\mu A^k\,\nabla_\mu A^{*\bar\ell}\,-\,F^k F^{*\bar\ell}\right)\cr
&+\ N_{\bar\imath j,k}\,F^{*\bar\imath}\,\left(\nabla^\mu A^k\,\nabla_\mu F^j\,
	-\,F^k\,\nabla^\mu\nabla_\mu A^j\right)\cr
&+\ N_{\bar\imath j,\bar\ell}\,F^j\,\left(
	\nabla^\mu F^{*\bar\imath}\,\nabla_\mu A^{*\bar\ell}\,
	-\,\nabla^\mu\nabla_\mu A^{*\bar\imath}\, F^{*\bar\ell}\right)\
    +\ \cdots .\cr
}\eqn\FthermsVIII
$$
Of particular importance is the first term here, which acts as a
kinetic-energy Lagrangian term for the auxiliary  --- or rather formerly
auxiliary and now propagating --- fields $F^i$ and $F^{*\bar\imath}$.
Consequently, the field equations for the $F^i$ now contain derivatives
of the $F^i$ themselves as well as of the $A^i$ fields:
$$
\eqalign{
g_{\bar\imath j}F^j\ ={}&
{\rm\DVIFeq}\ -\ \nabla^\mu\left( N_{\bar\imath j}\nabla_\mu F^j\
	+\ N_{\bar\imath j,\bar\ell}\,F^j\nabla_\mu A^{*\bar\ell}\right)\
    +\ N_{\bar\imath j,k}\nabla^\mu A^k\,\nabla_\mu F^j\cr
&+\ N_{\bar\imath j,k\bar\ell}\,F^j\nabla^\mu\, A^k\nabla_\mu A^{*\bar\ell}\
    -\ N_{\bar\imath j,k}\,F^k\,\nabla^\mu\nabla_\mu A^j\
    -\ N_{\bar\ell j,\bar\imath}\,F^j\,\nabla^\mu\nabla_\mu A^{*\bar\ell}\cr
&-\ (N_{\bar\imath j,k\bar\ell}+N_{\bar\ell j,k\bar\imath})F^j F^k F^{*\bar\ell}.\cr
}\eqn\DVIIIFeq
$$
Of course, \EightDerivatives\ gives just one example of an eight-super\-derivative
interaction; when all such interactions are taken into account, the field
equations for the $F^i$ fields become a really complicated mess.
But such details are not important for our argument;
what's important that the field equations for the $F^i$ --- and hence the
BPS equations~\val\BPSGeneric\ --- become very complicated differential
equations we do not know how to solve.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\APPENDIX{B}{B\break Proof of $X_1$--Dependence\break
 of the would-be Gaugino Condensate $S$ in MQCD}

In this Appendix we prove that all non-trivial solutions of eqs.~\val\EQPQ\
have $X_1$--dependent $S=PQ$ by assuming the contrary --- a solution with
$S=S(X_3)$ --- and showing that this solution must be trivial.
%
We begin by changing variables according to
$$
P\ =\ \sigma e^{+\gamma} ,\qquad Q\ =\ \sigma e^{-\gamma}
\eqno\eq
$$
where we assume $\sigma=\sqrt{S}$ to depend only on the $X_3$ and not on the
$X_1$.
Substituting these variables into eqs.~\val\EQPQ\ results in
$$
\eqalign{
Fe^{+\gamma}\left(\partial_3\sigma\,+\,\sigma\partial_3\gamma\right)\ &
=\ 0\ -\ i\sigma^*e^{-\gamma^*}\left(-\partial_1\gamma^*+\coeff1\N\right),\cr
Fe^{-\gamma}\left(\partial_3\sigma\,-\,\sigma\partial_3\gamma\right)\ &
=\ 0\ +\ i\sigma^*e^{+\gamma^*}\left(+\partial_1\gamma^*-\coeff1\N\right),\cr
}\eqno\eq
$$
where the $(c_1\partial_1+{ic_2\over\N})$ terms vanish because of
$J={-i\over\N}\partial_1(PQ)=0$.
A linear re-arrangement of eqs.~\? gives us
$$
\eqalign{
F\partial_3\sigma\ &
=\ +i\sigma^*\left(\partial_1\gamma^*-\coeff1\N\right)\,\cosh(\gamma+\gamma^*),\cr
F\sigma\partial_3\gamma\ &
=\ -i\sigma^*\left(\partial_1\gamma^*-\coeff1\N\right)\,\sinh(\gamma+\gamma^*)\cr
}\eqn\EQSG
$$
and hence
$$
{\partial_3\sigma\over\sigma}\
=\ -{\partial_3\gamma\over\tanh(\gamma+\gamma^*)}\, .
\eqn\KeyRatio
$$
The last equation is an ordinary differential equation with respect to the
$\partial_3$ and its real part can be easily integrated; this yields
$$
\sinh(\gamma+\gamma^*)\ =\ {h(X_1)\over|\sigma(X_3)|^2}
\eqn\GammaGamma
$$
for some $X_1$--dependent (but $X_3$--independent) integration ``constant'' $h$.
In light of the boundary conditions~\val\BoundaryConditions,
we should have $h=\sinh{2X_1\over\N}$, but out argument does not depend
on this specific form.

As a consequence of eq.~\GammaGamma, the coefficient $F$ in eqs.~\EQPQ\
and \EQSG\ depends only on the $X_1$ and not on the $X_3$.
Indeed,
$$
F\ \equiv\ 1\ +\ \coeff{1}{2\N}\partial_1(|P|^2-|Q|^2)\
=\ 1\ +\ {|\sigma|^2\over\N}\,\partial_1\sinh(\gamma+\gamma^*)\
=\ 1\ +\ {\partial_1 h(X_1)\over\N}\,.
\eqn\FXOne
$$

Next, consider the phase of $\partial_1\gamma^*-{1\over2\N}$.
According to the first eq.~\EQSG,
$$
\arg\left(\partial_1\gamma^*-\coeff1\N\right)\
=\ \arg(\partial_3\sigma/i\sigma^*) ,
\eqno\eq
$$
and since $\sigma$ does not depend on the $X_1$, the phase of the
$(\partial_1\gamma^*-\coeff1\N)$ should be $X_1$--independent as well.
In other words,
$$
\Im\partial_1\gamma\ =\ G(X_3)\left(\Re\partial_1\gamma-\coeff1\N\right)
$$
and
$$
\left(\partial_1\gamma^*-\coeff1\N\right)\
=\ \half(1-iG(X_3))\,\left(\partial_1(\gamma+\gamma^*)-\coeff2\N\right).
\eqno\eq
$$
Let us substitute the last formula into the first eq.~\EQSG.
After a little re-arrangement of factors, we obtain
$$
\eqalign{
{\partial_3\sigma^2(X_3)\over i+G(X_3)}\ &
=\ {|\sigma|^2\over F}\,\left[ \partial_1\sinh(\gamma+\gamma^*)\,
	-\,\coeff2\N\,\cosh(\gamma+\gamma^*)\right]\cr
&=\ {N\partial_1 h(X_1)\,-\,2\sqrt{h^2(X_1)+|\sigma(X_3)|^4}\over
	N\,+\,\partial_1 h(X_1)}\cr
}\eqn\Absurd
$$
where the left hand side should be $X_1$--independent but the right hand
side does depend on the $X_1$ for any non-trivial $h(X_1)\neq\rm const$.

By {\it reductio ad absurdum, Q.~E.~D.}

\endinput



==> Biblio.tex <==
%auto-ignore
%
% Bibliography for the DomainWall paper
%

\REF\KovShi {A.~Kovner and M.~Shifman \journal Phys. Rev. &D56 (1997) 2396--2402
	[hep-th/9611213].}

\REF\DvaShi {G.~Dvali and M.~Shifman \journal Phys. Lett. &396B (1997) 64--69
	and \jjournal \it ibid &407B (1997) 452 [hep-th/9612128].}

\REF\KovShiSmi {A.~Kovner, M.~Shifman and A.~Smilga
	\journal Phys. Rev. &D56 (1997) 7978--7989 [hep-th/9706089].}

\REF\Smilga{A.V.~~Smilga and A.~I.~Veselov \journal Phys. Rev. Lett. &79 (1997)
	4529--4532 [hep-th/9706217]
	\journal Nucl. Phys. &B515 (1998) 163--183 [hep-th/9710123]
	and \jjournal Phys. Lett. &428B (1998) 303--309 [hep-th/9801142];
	also A.~Smilga \journal Phys. Rev. &D58 (1998) 65 [hep-th/9711032].}

\REF\ShifmanI {M.~Shifman\journal Phys. Rev. &D57 (1998) 1258--1265
	[hep-th/9708060].}

\REF\ShifmanII {M.~Shifman and M.~Voloshin \journal Phys. Rev. &D57 (1998) 2590--2598
	[hep-th/9709137].}

\REF\Kovner {I.~Kogan,  A.~Kovner and M.~Shifman
	\journal Phys. Rev. &D57 (1998) 5195--5213 [hep-th/9712046].}

\REF\Matsuda {T.~Matsuda \journal Phys. Lett. &436B (1998) 264 [hep-th/9805134].}
% {\it ``On superpotential and BPS domain wall in SQCD and MQCD''.}   

\REF\CamHolWi {K.~Holland, A.~Campos and U.~J.~Wiese
	\journal Phys. Rev. Lett. &81 (1998) 2420--2423 [hep-th/9805086].}

\REF\VenYan {G.~Veneziano and S.~Yankielowicz \journal Phys. Lett. &113B (1982) 231.}

\REF\TVY {T.~R.~Taylor, G.~Veneziano and S.~Yankielowicz
	\journal Phys. Lett &113B (1982) 231
	and \jjournal Nucl. Phys. &B218 (1983) 493.} 

\REF\AffDinSei {I.~Affleck, M.~Dine and N.~Seiberg
	\journal Nucl. Phys. &B241 (1984) 493
	and \jjournal Nucl. Phys. &B256 (1985) 557. }

\REF\sw {N.~Seiberg and E.~Witten \journal Nucl. Phys. &B426 (1994) 19--52
	 \hbox{[hep-th/9407087]\kern -3pt}\penalty -5000
%``Electric-Magnetic Duality,
%Monopole Condensation, And Confinement In $N=2$ Supersymmetric
%Yang-Mills Theory", 
	and \jjournal Nucl. Phys. &B431 (1994) 484--550 [hep-th/9408099].}
%``Monopoles, Duality, And Chiral
%Symmetry Breaking In $N=2$ Supersymmetric QCD", 

\REF\WittenMQCD {E. Witten \journal Nucl. Phys. &B500 (1997) 3--42
	[hep-th/9703166].}
%``Solutions of Four-Dimensional Field Theories via $M$ Theory",

\REF\HOO {K.~Hori, H.~Ooguri, Y.~Oz
	\journal Adv. Theor. Math. Phys. &1 (1998) 1--52 [hep-th/9706082].}
%``Strong Coupling Dynamics of Four-Dimensional N=1 Gauge Theories
% from M Theory Fivebrane"

\REF\WittenQCD {E.~Witten \journal Nucl. Phys. &B507 (1997) 658--690
	[hep-th/9706109].}
%``Branes and the Dynamics of QCD", 
%\let\wittenQCD=\WittenQCD

\REF\Volovich {A.~Volovich, hep-th/9801166.}
% ``Domain walls in MQCD and Monge-Ampere equation"

\REF\MAbook {Thierry Aubin, {\it ``Non Linear Analysis on Manifolds,
	Monge-Ampere Equations,''} Springer-Verlag, New York,  Heidelberg, Berlin, 	1982}

\REF\LouKap{V.~Kaplunovsky and J.~Louis \journal Nucl. Phys. &B422 (1994) 57--124
	[hep-th/9402005].}

\REF\IntSei{K.~Intriligator and N.~Seiberg
	\journal Nucl. Phys. &B431 (1994) 551--568 [hep-th/9408155].}

\REF\biksy {A.~Brandhuber, N.~Itzhaki, V.~Kaplunovsky, J.~Sonnenschein and\brk
	S.~Yankielowicz \journal Phys. Lett. &410 B (1997) 27--35 [hep-th/9706127].}
%``Comments on the M Theory Approach to N=1 SQCD and Brane Dynamics",

\REF\bbs {K.~Becker, M.~Becker and A.~Strominger
	\journal Nucl. Phys. &B456 (1995) 130 [hep-th/9507158].}
%``Fivebranes, Membranes, And Nonperturbative String Theory"

\REF\bbmooy {K.~Becker, M.~Becker, D.~R.~Morrison, H.~Ooguri, Y.~Oz and Z.~Yin
	\journal Nucl. Phys. &B480 (1996) 225 [hep-th/9608116].}
%``Supersymmetric Cycles in Exceptional Holonomy Manifolds and Calabi-Yau 4-Folds",

\REF\joyce {D.~Joyce \journal Jour. Diff. Geom. &43 (1996) 291 and
	\jjournal Jour. Diff. Geom. &43 (1996) 329.}
% ``Compact Riemannian 7-Manifolds With Holonomy $G_2$. I"
%``Compact Riemannian 7-Manifolds With Holonomy $G_2$. II"

\REF\lean {R.~C.~McLean, {\it ``Deformations of calibrated submanifolds,''}
	DUK--M--96--01, \href{http://www.math.duke.edu/preprints/96-01.dvi}%
	{http://www.math.duke.edu/preprints/96-01.dvi}.}
%\jdg{?}{?}{?}, preprint available at

\REF\Oraigh {L.~O'Raighfeartaigh \journal Nucl. Phys. &B96 (1975) 331.}

\REF\KLT {A.~Klemm, W.~Lerche and S.~Theisen
	\journal Int. Jour. Mod. Phys. &A11 (1996) 1929--1974 [hep-th/9505150].}
%``Nonperturbative effective actions for $N=2$ supersymmetric gauge theories"

\REF\DS {M.~R.~Douglas and S.~H.~Shenker \journal Nucl. Phys. &B447 (1995) 271--296
	[hep-th/9503163].}


\endinput


==> GauginoCond.tex <==
%auto-ignore
%
% Chapter 6 of the DomainWall paper
%
\chapter{Gaugino Condensates and Effective Superpotentials}
%
When the scalar field $\Phi$ is light, its condensate $U=\vev{\tr\Phi^2}$
dominates the low-energy dynamics of the softly broken $\NS=2$ SSYM
theory, hence the success of the SW theory whose primary focus is on
the $U$ dependence of various quantities.
The low-energy importance of $\Phi$ and $U$ diminishes with $\Phi$'s mass
$m$; in the large $m$ limit, $\Phi$ and one of the two gauginos decouple
leaving us with an effective $\NS=1$ SSYM theory with
$$
\Lambda_{\rm eff}\ \equiv\ \Lambda_1\ =\ \root 3\of{-m\Lambda^2_2\,}.
\eqn\LambdaOneTwo
$$
(In this section we refer to the $\Lambda$ parameter of the
high-energy $\NS=2$ SSYM theory
as $\Lambda_2$ in order to to distinguish it from the $\Lambda_1$.)
This effective $\NS=1$ SSYM theory has $\N$ isolated vacua related
to each other by a spontaneously broken $Z_\N$ symmetry;
the order parameter distinguishing between the vacua is the
{\sl gaugino condensate}\refmark\VenYan\
$$
S\ \equiv\ \coeff{1}{16\pi^2}\vev{\tr\lambda^\alpha\lambda_\alpha}\
=\ \Lambda_1^3\,e^{2\pi i n/\N} ,\quad
n=1,2,\ldots,\N.
\eqn\GCondensate
$$
{}From the infrared point of view, $S$ is the scalar component of the composite
chiral superfield $\coeff{1}{16\pi^2}\tr(W^\alpha W_\alpha)$ describing the
lightest glueballs/oddballs of the SSYM theory.
Integrating out all the heavier particles leaves us with an effective theory
for the gaugino condensate $S$.
The Veneziano--Yankielowicz superpotential\refmark\VenYan\
$$
W(S)\ =\ S\,\log{S^\N\over (e\Lambda_1^3)^N}
\eqn\VYT
$$
of this theory is exact --- it is completely determined by the R-anomaly of the SSYM
--- but multi-valued (the logarithm is only defined modulo $2\pi i$);
altogether, it has $\N$ supersymmetric vacua~\GCondensate.

For our purpose of constructing BPS domain wall solutions, the
Veneziano--Yankielowicz--Taylor\refmark\TVY\  effective theory of the gaugino condensate $S$
has two major deficiencies.
First, as argued by Kovner and Shifman,\refmark\KovShi different vacua~\GCondensate\
belong to different branches of the multi-valued superpotential~\VYT,
which means that additional, heavier degrees of freedom become excited
%--- and must be accounted for ---
in the mid-wall region of space where
$W_{\rm eff}(S(x_3))$ jumps from one branch of \VYT\ to another.
Without somehow accounting for such heavier degrees of freedom
we would have an apparent discontinuity of $W(x_3)$ and hence an
unresolved singularity of the energy density of a BPS domain wall
$$
{d\,{\rm Energy}\over d\,{\rm Volume}}\
=\ 2\left|{dW\over dx_3}\right| .
\eqn\BPSLocal
$$
This problem becomes particularly severe in the large $\N$ limit
where this singularity accounts for almost all of the wall's energy;
this problem is discussed in great detail in refs.~[\KovShiSmi] and we have nothing
to add to {\sl that} discussion in this article.

On the other hand,
for $\N=2$ the superpotential $W(S(x_3))$ is actually continuous:
Indeed, both vacua $S=-\Lambda_1^3$ and $S=+\Lambda_1^3$
of the $SU(2)$ SSYM are invariant under the charge conjugation symmetry
of the theory,
\foot{Without loss of generality, we assume real $\Lambda_1^3>0$.}
$S\to S^*$.
The entire domain wall solution is therefore C-invariant, \ie,
real $S(x_3)$ throughout the wall;
the superpotential $W(S(x_3))$ is given by the real branch of~\VYT\ for real $S>0$
for $x_3<0$ and by a different branch that is real for real $S<0$
for $x_3>0$, but both branches have $W=0$ for $S=0$ at $x_3=0$.
Thus we have no discontinuity and the two branches of
the $W(S(x_3))$ account
for the entire energy of the BPS domain wall.

The other major difficulty with the Veneziano--Yankielowicz--Taylor
\refmark\TVY\ theory
is that it does not provide us with an effective K\"ahler function
for the gaugino condensate, never mind the higher-derivative
terms in the effective low-energy Lagrangian.
{}From the SSYM point of view, even the K\"ahler term
$\int\!d^4\theta\,K(S,\overline S)$ is a high-derivative term in the gauge theory's
generating functional $\Gamma$ and hence subject to all kinds of perturbative
and non-perturbative corrections.
Thus, the derivative interactions of the $S$ superfield remain quite unknown
\foot{Qualitatively, we expect the K\"ahler metric $g_{S\overline S}$
	to be non-singular --- otherwise, contrary to Witten's supersymmetric
	index theorem,
	there would be extra supersymmetric vacua in addition to \GCondensate.
	(Actually, a chirally invariant vacuum with a massless fermion at $S=0$
	would be consistent with the Witten's index, but
	contrary to some statements in the literature,\refmark{\KovShi-\Smilga}
	there are no
	physical reasons for the existence of such a vacuum.)
	Unfortunately, K\"ahler functions of $\NS=1$ theories are not related
	to holomorphic functions (such as prepotentials of $\NS=2$ theories),
	so absence of singularities is not much of a constraint.}
%
and because of this lack of crucial data, we have no way of calculating the actual
profile $S(x_3)$ of the BPS domain wall configuration, not even for $\N=2$.
All we can say with confidence is that the overall thickness $w$ of the wall
should be of the order $O(1/|\Lambda_1|)$ (give or take a power of the~$\N$),
simply because it's the only distance scale of the $\NS=1$ SSYM theory.

\par\smallskip
\line{\hfil$*$\quad$*$\quad$*$\hfil}
\smallskip

Let us now turn our attention to the regime of $m\sim\Lambda_2\sim\Lambda_1$
when both gaugino condensate and scalar condensates are equally important.
For $\N=2$, the only gauge-invariant condensate of the adjoint field $\Phi$
is $U=\vev{\tr\Phi^2}$ and the Veneziano--Yankielowicz--Taylor
superpotential\refmark\TVY\ for the $S$ and $U$ condensates
is completely determined by the
global $U(1)_A\times U(1)_R$ symmetries of the $\NS=1$ gauge theory and their
anomalies,\refmark{\LouKap,\IntSei}
$$
W(S,U)\ =\ S\,\log{U^2\over\Lambda_2^4}\ +\ mU .
\eqn\VYTSU
$$
Again, this superpotential has infinite number of branches but only two
physically distinct supersymmetric vacua:
$$
\eqalign{
1)\quad & U\ =\ +\Lambda^2_2\,,\quad
	S\ =\ -m\Lambda^2_2\ =\ +\Lambda_1^3\,,\quad W\ =\ +m\Lambda_2^2\,,\cr
2)\quad & U\ =\ -\Lambda^2_2\,,\quad
	S\ =\ +m\Lambda^2_2\ =\ -\Lambda_1^3\,,\quad W\ =\ -m\Lambda_2^2\,.\cr
}\eqn\TwoVYTVacua
$$
The superpotential~\VYTSU\ is exact, thus the two vacua~\TwoVYTVacua\ persist
for all non-zero values of the mass parameter $m$.
Indeed, for small $m\ll\Lambda_2$, the two vacua
\val\SWConfiningVacuum\ and \val\SWObliqueVacuum\ of the Seiberg--Witten
theory are in exact agreement with the eqs.~\TwoVYTVacua;
likewise, the two vacua~\GCondensate\ of the effective pure-gauge $SU(2)$
SSYM theory for large $m\gg\Lambda_2$ also agree with the \TwoVYTVacua.

Unfortunately, the
Veneziano--Yankielowicz--Taylor theory does not provide us with a
K\"ahler function $K(S,U,\overline S,\overline U)$ or any knowledge of the
higher-derivative interactions of the $S$ and $U$ superfields.
Consequently, we are unable to calculate the field profiles $S(x_3)$ and
$U(x_3)$ for the domain wall solution interpolating between the two vacua
\TwoVYTVacua.
Nevertheless, we can make a qualitative statement:
{\sl There should be BPS-saturated domain wall solutions for all $m\neq0$.}
Indeed, we know that such solutions do exist in the Seiberg--Witten regime
of small $m\ll\Lambda_2$, \cf\ section~4.
We do not know what exactly happens in the $m\gsim\Lambda_2$ regime, but if
a BPS saturated wall were to suddenly 
disappear at some finite value of the $m/\Lambda_2$
ratio, it would mean some kind of a discontinuous phase transition.
On the other hand, the vacuum structure~\TwoVYTVacua\ smoothly continues
for all $m\neq0$, which strongly militates against any discontinuities
at finite $m/\Lambda_2$.
Although this is not a rigorous proof of existence of BPS saturated walls
at large $m$ (and hence all $m\neq0$),
it is a very strong argument in their favor.

\par\smallskip
\line{\hfil$*$\quad$*$\quad$*$\hfil}
\smallskip

We conclude this section with a discussion of the three gaugino species
in the $SU(2)$ gauge theory with an adjoint scalar,
namely the electrically neutral
`photino' $\lambda^{(0)}_\alpha$ and the charged `winos' $\lambda^{(\pm)}_\alpha$.
Because of the gauge symmetry,
the distinction between the gaugino species arises from the scalar field:
For example, the photino field can be identified in
gauge invariant terms as
$$
\lambda^{(0)}_\alpha\
\buildrel {\scriptscriptstyle\rm def}\over=\ 
{\tr(\lambda_\alpha\,\Phi)\over\sqrt{U}}\,.
\eqn\Photino
$$
Notice that according to this definition, $\lambda_0^\alpha$ is the lowest
component of a gauge-invariant chiral superfield
$\tr(W^\alpha\Phi)/\sqrt{U}$, which belongs to the chiral ring of the
$\NS=1$ theory.
Therefore, {\sl in any supersymmetric vacuum} of the theory,
$$
\vev{\lambda^{(0)\alpha}\,\lambda^{(0)}_\alpha}\
=\ \vev{\lambda^{(0)\alpha}}\vev{\lambda^{(0)}_\alpha}\ \equiv\ 0.
\eqn\PhotinoCond
$$
Thus, {\sl the photinos do not form a condensate} and
the net gaugino condensate $S$ is actually the wino condensate
$S^\pm=\coeff{1}{16\pi^2}\vev{\lambda^{(+)\alpha}\,\lambda^{(-)}_\alpha}$.

The theorem \PhotinoCond\ assumes all four supercharges of the $\NS=1$
theory remain unbroken in the vacuum state;
it does not apply to BPS-saturated field configurations that leave two
of the supercharges unbroken but break the other two.
Consequently, no theorem prohibits the {\sl local}
photino condensate field
$S^0(x)=\coeff{1}{32\pi^2}
\vev{\lambda^{(0)\alpha}(x)\,\lambda^{(0)}_\alpha(x)}$
{}from acquiring non-zero values within a BPS-saturated domain wall.
The only general rules are $S^0(x_3)\to 0$ for $x_3\to\pm\infty$ ---
in the vacuum domains on either side of the wall, the photino condensate
must vanish --- and $S^0(x_3=0)=0$ following from
the $Z_2$ symmetry of the domain wall.
Figure~6\figinsert{f6}
illustrates a generic photino-condensate profile $S^0(x_3)$
consistent with these rules.

Of course, just because a non-zero photino condensate is allowed to exist
within a BPS domain wall, no theorem requires its actual presence.
In order to show that the photino condensate is indeed present within the wall,
let us consider the Seiberg--Witten limit $m\ll\Lambda_2$.
In the perturbed Coulomb phase prevalent throughout most of the SW wall,
the only light fields are the scalar $U$, its superpartner $\psi$, the photon
and the photino $\lambda^{(0)}$, all governed by the effective component-field Lagrangian
$$
\eqalign{
{\cal L}\ &
=\ g^{U\overline U}\left( |\partial_\mu U|^2\,
	+\,\coeff{i}{2}\bar\psi\!\not\!\!D\psi\,
	+\,\left|m+{i\over16\pi}\,{d\tau\over dU}\,
		\lambda^{(0)}\lambda^{(0)}\right|^2
	\right)\cr
&\quad+\ {1\over4\pi\Im\tau}\left(\coeff14 F_{\mu\nu}^2\,
	+\,\coeff{i}{2}\bar\lambda^{(0)}\!\not\!\!D\lambda^{(0)}\,
	+\,\coeff14\left|{d\tau\over dU}\,\lambda^{(0)}\psi\right|^2
	\right)\cr
&\quad+\ {i\over16\pi}\,{d^2\tau\over dU^2}\,(\lambda^{(0)}\lambda^{(0)})\,(\psi\psi)\
	+\ \rm H.\,c.\cr
}\eqn\CoulombLagrangian
$$
Of particular interest to us is the fermionic mass term
$$
{\cal L}_{\rm mass}\
=\ {im^*\,g^{U\overline U}\over16\pi}\,{d\tau\over dU}\,\lambda^{(0)}\lambda^{(0)}\
+\ {\rm H.\,c.}\
=\ {-i\over16\pi}\,{d\tau(U)\over dx_3}\,\lambda^{(0)}\lambda^{(0)}\
+\ {\rm H.\,c.}
\eqn\PhotinoMass
$$
(\cf\ eq.~\val\SWCoulombPhase):
Inside a BPS domain wall, the photino has a (position-dependent) Majorana mass.
Consequently, at the one-loop level of the effective theory, we have the photino
condensate
$$
\vev{\lambda^{(0)}\lambda^{(0)}}(x)\
=\ \lim_{x'\to x}\bra{x}\,\tr({\rm photino\ propagator})\,\ket{x'}\ \neq\ 0.
\eqn\PhotinoCondensate
$$
Unfortunately, the ultraviolet limit here diverges quadratically as
$m/(x'-x)^2$.
Of course, in the full theory this divergence is somehow cut off at the strong
interaction scale $\Lambda_2$, thus
$$
S^0(x_3)\Bigr|_{\rm wall}\ = O(m\Lambda_2^2),
\eqn\SEstimate
$$
but without detailed knowledge of this effective cutoff we are unable to
calculate the actual profile $S^0(x_3)$ of the photino condensate.

Finally, a few words about the winos and the wino condensate $S^\pm(x_3)$.
In the massless Seiberg--Witten theory,
the winos belong to short vector multiplets $W^\pm$
of the $\NS=2$ supersymmetry and their physical mass saturates the BPS
limit, $M_W=2|A_1(U)|$, \cf~eq.~\val\EllipticCurve.
As argued in refs.~[\sw], there is a circle-like line in the complex $U$ plane
defined by the marginal-stability condition
$$
\Im\bigl(A_1^*(U)\,A_2(U)\bigr)\ =\ 0.
\eqn\MarginalStability
$$
Outside this line (\ie, for sufficiently large $U$), the $W^\pm$ multiplets are
stable, but they become marginally unstable along the line~\MarginalStability\
and disappear from the particle spectrum for small $U$ inside the line.
In the field-theoretical terms, the kinetic energies of the $W^\pm$ fields
become negative for the values of $U$ inside the line~\MarginalStability.
In a massive SW theory, there are corrections to kinetic energies of various fields
due to the $\NS=2$ breaking mass $m$;
thus we expect $O(m)$ corrections to the location of the marginal stability line
for the $W^\pm$ vectors and winos.
Indeed, the two vacua \val\SWConfiningVacuum\ and \val\SWObliqueVacuum\ of the massive
SW theory lie directly atop the massless marginal stability line~\MarginalStability,
but the winos are actually stable enough to form the wino condensates
$S^\pm=\pm m\Lambda_2^2$ (\cf~eq.~\TwoVYTVacua).
Altogether, for small but non-zero masses $m$,
the stability region of the winos should look like
the dark-grey area on figure~7.\figinsert{f7}

Now consider a SW domain wall where the $U$ field smoothly changes
from $+\Lambda^2_2$ to $-\Lambda_2^2$.
Through most of the wall's interior region, $U(x_3)$ traverses the dark grey
region of figure~7 where the particle spectrum of the theory does not contain
the $W^\pm$ vector bosons and their wino superpartners.
For small $m$, we may neglect the effects of a small gradient of the $U$ field
on the wino kinetic energy, thus {\sl through most of the domain wall's
interior, winos do not exist and there is no wino condensate.}
However, near either end of the domain wall, $U(x_3)$ crosses into the white
region of figure~7 where the winos do exist and presumably do form a condensate.
Indeed, the wino condensate $S^\pm(x_3)$ must exist and asymptote to $\pm m\Lambda_2^2$
for $x\to\pm\infty$ since these are the vacuum values of the net gaugino condensate
$S=S^\pm+S^0$ while the photino condensate $S^0$ has to asymptote to zero
as one goes into the domain of a stable $\NS=1$ vacuum,
\cf\ eq.~\PhotinoCond\ and figure~6.
To summarize, figure~8\figinsert{f8}
shows the qualitative behavior of the wino and photino
condensates in the Seiberg--Witten regime ($m\ll\Lambda_2$) of the BPS domain wall.

In the large $m\gsim\Lambda_2$ regime of the BPS domain wall,
the gaugino condensates behave quite differently.
In the extreme $m\gg\Lambda_2$ --- and hence $m\gg\Lambda_1\gg\Lambda_2$ --- regime,
the scalar field $\Phi$ decouples, its expectation value becomes unimportant
and the distinction between the photino and the winos becomes unphysical.
(Formally, as long as $U\neq0$, we may define a ``photino'' field
according to eq.~\Photino, but the physical meaning of such definition becomes rather
obscure when $|U|\ll\Lambda_1$).
Consequently, only the net gaugino condensate $S(x_3)$ is meaningful in this regime.

On the other hand, for $m\sim\Lambda_2$ we can readily distinguish the photinos
from the winos.
At the same time however, there are large $m$-dependent corrections to the SW
formul\ae\ for the kinetic energies of the $W^\pm$ and wino fields, so it is
quite possible that these fields exist throughout the domain wall, including
the $U\approx0$ region in the wall's middle.
If this is indeed the case, we expect both the photino and the wino condensates
to be present throughout the wall but to follow different profiles,
$S^\pm(x_3)\neq S^0(x_3)$.
As of this writing, our knowledge of this regime is limited to generalia;
this is a subject for future research.

\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







==> Intro.tex <==
%auto-ignore
%
% Chapter 1 of the DomainWall paper
%
\chapter{Introduction}
%
Domain walls interpolating between degenerate discrete vacua
have been a subject of a rather intensive study in recent years.
\refmark{\KovShi-\CamHolWi}
In particular, an $\NS=1$ Supersymmetric
$SU(\N)$ Yang--Mills theory has a non-anomalous $Z_{2\N}$ chiral
symmetry which is spontaneously broken down to the $Z_{2}$
by the expectation
value of the gaugino bilinear $\vev{\tr\lambda^\alpha\lambda_\alpha)}$.
The SSYM theory thus has $\N$ degenerate discrete vacua,
each characterized by a
different value of the chiral gaugino condensate\refmark\VenYan\
$$
\vev{\tr\lambda^\alpha\lambda_\alpha}\
=\ 16\pi^2\Lambda^3\,e^{2\pi i n/\N},\quad n=1,2,\ldots,\N.
\eqn\NVacua
$$
Of special interest are the so-called BPS-saturated domain walls
which preserve half of the $\NS=1$ supersymmetry.
Fields configurations for such BPS-saturated walls satisfy first-order
differential equations, which follow in a straightforward manner from
the effective Lagrangian of the theory.
Like other BPS-saturated states, the BPS domain wall are more tractable
and one may reasonably hope for some exact results for such walls even
in a context of a confining strongly interacting theory.
Indeed, the tension \ie\  energy per unit area of a BPS domain wall is
exactly determined by the difference between the superpotential values
in the two vacua connected by the wall.
In the $\NS=1$ SSYM theory, the superpotential --- which acts as a
central charge for domain walls --- is related by the chiral
anomaly to the gaugino condensate, so a BPS domain wall 
has tension\refmark\DvaShi
$$
{\cal T}\ \equiv\ {\rm Energy\over Area}\ =\ {\N\over 8\pi^2}\,
\bigl| \Delta\vev{\tr\lambda^\alpha\lambda_\alpha}\bigr| .
\eqn\Tension
$$

For the $\NS=1$ SQCD theories with $N_f<\N$, the effective superpotential
is so constrained by the twin requirements of the holomorphy
and flavor symmetry that one can completely determine
its exact form.\refmark{\VenYan,\TVY,\AffDinSei}\ 
Unfortunately, no such constraints apply to the effective K\"ahler function
of the theory which controls the kinetic energies of the fields.
The K\"ahler metric of the field space plays important role in the BPS
equations, so the very existence of BPS-saturated domain walls is
a non-trivial dynamical question.
Thus far, all the investigations of this issue have {\sl assumed} specific
K\"ahler functions, only to find that the answer depends
on their assumptions.
Furthermore, the singularities of the K\"ahler metric can lead to additional
vacuum states of the theory;
indeed, the claims\refmark{\KovShi-\Smilga}\  
that SQCD may have a chirally-invariant vacuum
are based on precisely such a K\"ahler singularity.

The situation is under much better control for the $\NS=2$ SQCD
where the K\"ahler metric follows from a holomorphic pre-potential
and the entire low-energy effective Lagrangian is completely
determined by the Seiberg--Witten theory.\refmark\sw\
In the $\NS=1$ terms, the $\NS=2$ SQCD has an extra chiral superfield
in the adjoint representation of the gauge group.
Giving this superfield a mass $m\neq0$ breaks the supersymmetry down to
$\NS=1$; in the $m\to\infty$ limit, the adjoint superfield decouples
from the low-energy physics and one is left with an effective
$\NS=1$ SQCD.
We have therefore decided to study the BPS-saturated domain walls
in the $\NS=2$ SQCD perturbed by the adjoint mass $m$.
For the sake of simplicity, we focus on the $SU(2)$ SSYM theory
without any quarks.
An overview of the $SU(2)$ Seiberg--Witten (SW) theory perturbed by the
adjoint mass is presented in section~2 of this article;
we emphasize the vacuum structure of the theory.

In section 3, we discuss BPS-saturated domain walls in a
toy model with a simplified version of the Seiberg--Witten superpotential
and a naive \ie, flat K\"ahler metric.
Also the electric and the magnetic charges of the SW theory are replaced
with two purely electric charges of an $U(1)\times U(1)$ gauge theory.
We write down the BPS equation for a domain-wall field configuration
and solve them analytically for a particular value of the mass parameter
and numerically otherwise.
It turns out that in the small mass limit (analogous to $m\ll\Lambda$),
the domain wall's profile develops a sandwich-like five-layer structure.
In each of the two outer layers, the fields asymptote to their respective
vacuum values and one combination of the two $U(1)$ charges is Higgsed
down; this behavior corresponds to the two confining phases of the SW theory
characterized by respectively magnetic monopole or dyon condensates.
In the middle layer, the toy model is in its Coulomb phase, the
$U(1)\times U(1)$ gauge symmetry is essentially unbroken and the modulus
field slowly interpolates between its stable-vacuum values;
for $\rm mass\neq0$, the Coulomb phase is thermodynamically unstable in 
the bulk 
but exists in a layer of finite thickness inside the domain wall.
The two remaining layers contain transition regions between the Coulomb
and the appropriate confining phases.

Section 4 of this article is devoted to the analysis of BPS domain walls
in Seiberg--Witten theory with a small adjoint mass $m\ll\Lambda$.
We argue that in the small mass regime, the SW domain wall has the
same five-layer structure as the toy model. We write down the BPS
equations for each of the wall's layers and we solve those equations
numerically.
We find a surprisingly low limit $m\lsim\Lambda/400$ for the clear
five-layer structure of the SW domain wall; beyond this limit,
the transition regions take over the Coulomb phase region and overlap
each other.
Also, the wall becomes too thin to be analyzed in terms of a low-energy
\ie\ long-distance effective theory such as Seiberg--Witten;
this problem is discussed in section~5.
%
Nevertheless, we shall argue that the BPS-saturated domain wall
exists for any $m$, small or large.

In section 6 we discuss gaugino condensation in the Seiberg--Witten theory.
We write down an effective superpotential and analyse the vacuum structure
of the theory in terms of both gaugino and scalar condensates.
We find the same two stable vacua for all $m\neq0$ and no trace of any
additional chirally invariant vacuum.
We also deduce the qualitative behavior of the gaugino condensates inside
the domain wall.
For finite $m$, there are distinct ``photino'' and ``Wino'' condensates
and their profiles inside the wall are quite different.

E.~Witten\refmark\WittenMQCD\ has advocated the MQCD approach based on
the M--theory.
Hopefully, the $\NS=1$ MQCD is in the same universality class as the
ordinary $\NS=1$ SQCD.
In MQCD, the BPS-saturated domain walls arise naturally and have a
geometric interpretation;\refmark\WittenQCD\ there is even a geometric interpretation
of the QCD string emanating from a probe quark and
terminating on the wall.
Witten argues that in the large $\N$ limit, the BPS wall's tension
should scale as ${\cal T}\propto\N$,\refmark\WittenQCD which makes it hard to interpret
the wall as a soliton in the effective low-energy theory since
the tension of such a solitonic wall would scale as ${\cal T}\propto\N^2$.
\foot{See however [\Kovner] for efforts to explain the ${\cal T}\propto\N$
	scaling behavior in the field theory framework.}

In section 7, we follow Witten's geometric construction of a BPS domain
wall in MQCD and write down explicit BPS equations for the wall's
geometry.
The equations are rather cumbersome, although we managed to simplify them
 and recast them as a pair of partial differential equations
for two complex functions.
In the $SU(2)$ case, the two functions are actually real and the BPS
equations can be further reduced  to a single fourth-order
Monge--Ampere equation\refmark{\Volovich,\MAbook}
for one real function.
Unfortunately, we were unable to find an analytic solution compatible
with the domain-wall boundary conditions.
We also present simplified equations for the MQCD analogue of the
low-mass Seiberg--Witten domain wall; again, we do not have a
solution.
We hope however that someone will eventually solve our equations;
such a solution would be very useful for studying many physical properties
of the domain walls in MQCD --- and ultimately, in QCD itself. 

\endinput


==> MQCD.tex <==
%auto-ignore
%
% Chapter 7 of the DomainWall paper
%
\chapter{BPS Domain walls in MQCD}
%
In this last section of the paper, we shift our focus from the supersymmetric
gauge theory to another theory in the same universality class, namely
the MQCD.\refmark\WittenMQCD
Generally, MQCD is a geometric theory of the M5-brane of the M-theory living in
space of geometry ${\bf R}^{1,3}\otimes {\cal Y}^7$ and completely spanning
the ordinary four-dimensional spacetime~${\bf R}^{1,3}$.
For the vacuum states of MQCD, the M5-brane geometry\refmark{\WittenQCD,\HOO\biksy}
 is ${\bf R}^{1,3}\otimes \Sigma$
for some Riemann surface $\Sigma\subset{\cal Y}^7$;
different vacua have different Riemann surfaces $\Sigma'\neq\Sigma$.
The non-vacuum solutions have $M5={\bf R}^{1,3}\times\Sigma(x_0,x_1,x_2,x_3)$;
in particular, a domain-wall solution has $x_3$-dependent $\Sigma(x_3)$
interpolating between two vacua $\Sigma_1$ and $\Sigma_2$.
In other words,
$$
M5\ =\ {\bf R}^{1,2}\otimes\SS,
\eqno\eq
$$
where $\SS\subset{\bf R}_{x_3}\otimes{\cal Y}^7$
is a three-cycle with boundaries $\Sigma_1$ at $x_3=-\infty$
and $\Sigma_2$ at $x_3=+\infty$.

Supersymmetry requires ${\cal Y}^7={\cal Y}^6\otimes{\bf R}$
where ${\cal Y}^6$ is a K\"ahler space;
for the problem at hand, ${\cal Y}^6={\bf R}^5\otimes S^1$
is actually flat.
The supersymmetric vacua correspond to the supersymmetric 2--cycles of the ${\cal Y}^6$
\ie, the Riemann surface $\Sigma$ should be holomorphically embedded into the
${\cal Y}^6$.
Likewise, BPS-saturated domain walls that preserve two unbroken supercharges
correspond to the supersymmetric 3--cycles \ie, {\sl associative submanifolds}
$\SS\subset{\bf R}_{x_3}\otimes{\cal Y}^6$.\refmark{\bbs,\bbmooy}
The associativity condition is best explained\refmark{\joyce,\lean}
in terms of a $G_2$ structure
of the ${\bf R}_{x_3}\otimes{\cal Y}^6$ manifold, namely the invariant 3--form
$$
\phi\
=\ \coeff{i}{2}\,dx_3\wedge\left( dz_1\wedge d\bar z_1 + dz_2\wedge d\bar z_2
			+dz_3\wedge d\bar z_3 \right)\
+\ \Im\left( dz_1\wedge dz_2\wedge dz_3 \right)
\eqn\ThreeForm
$$
where $(z_1,z_2,z_3)$ --- collectively denoted $\vec z$ ---
 are the complex coordinates of the ${\cal Y}^6$.
The volume form (for the induced Riemannian metric) of any 3--cycle of such
a manifold is limited from below by the pull-back of the 3--form~\ThreeForm;
the associative 3--cycles saturate this lower bound
and hence have lowest volumes allowed by their topologies and boundary conditions.
(This is similar to the holomorphic 2--cycles of a K\"ahler manifold having
lowest areas allowed for their topologies and boundary conditions.)

Specifically, let $X_1$, $X_2$ and $X_3$ be generic world-volume coordinates
of the 3--cycle $\SS$ and let $\alpha_i=dx_3/dX_i$ and $\vec a_i=d\vec z/dX_i$.
In terms of these derivatives, the pull-back of the 3--form~\ThreeForm\ is
$$
\phi_{\rm pb}\ =\ \hat\phi\,dX^1\wedge dX^2\wedge dX^3\quad
{\rm where}\ \hat\phi\ =\ \Re\left[(\vec a_1\times \vec a_3)\cdot\vec a_3\right]\
+\ \half\epsilon_{ijk}\,\alpha_i\Im\left[{\vec a}_j^*\cdot\vec a_k\right]
\eqn\PullBack
$$
while the volume form is of course
 $V=\sqrt{\det(h)}\,dX^1\wedge dX^2\wedge dX^3$ for
the induced metric
$$
h_{ij}\ =\ \alpha_i\alpha_j\ +\ \Re\left[{\vec a}_i^*\cdot\vec a_j\right].
\eqn\MetrichIJ
$$
Given these formul\ae, straightforward but tedious algebra yields
$$
\det(h_{ij})\ -\ \hat\phi^2\
=\ \left|\vec R\right|^2\ +\ \Im^2\left[(\vec a_1\times \vec a_3)\cdot\vec a_3\right]
\eqn\Lemma
$$
where
$$
\vec R\ =\ \half\epsilon_{ijk}\left[ \alpha_i\,(\vec a_j\times\vec a_k)\
	-\ {\vec a}^*_i\,({\vec a}_j^*\cdot\vec a_k)\right]\,;
\eqn\Rdef
$$
furthermore, $\vec R=0$ implies
$\Im\left[(\vec a_1\times \vec a_3)\cdot\vec a_3\right]=0$.
Therefore, {\it a 3--cycle is associative and the domain wall is BPS saturated
if and only if $\vec R=0$.}

In order to make practical use of this theorem, let us choose the world-volume
coordinates according to
$$
X^1\, +\, iX^2\ =\ z^3,\qquad X^3\ =\ x^3
\eqno\eq
$$
which gives us
$$
\eqalign{
\alpha_1\ =\ 0, &\qquad \vec a_1\ =\ (\partial_1 z_1,\partial_1 z_2,1),\cr
\alpha_2\ =\ 0, &\qquad \vec a_2\ =\ (\partial_2 z_1,\partial_2 z_2,i),\cr
\alpha_3\ =\ 1, &\qquad \vec a_3\ =\ (\partial_3 z_1,\partial_3 z_2,0).\cr
}\eqn\Derivatives
$$
%and hence
%$$
%\vec R\ =\ \vec a_1\times\vec a_2\ -\ \vec a_3^*\,\Im[\vec a_1^*\cdot\vec a_2]\
%-\ \vec a_1^*\,\Im[\vec a_2^*\cdot\vec a_3]\ -\ \vec a_2^*\,\Im[\vec a_3^*\cdot\vec a_1].
%\eqn\RR
%$$
In light of these formul\ae, the $\vec R=0$ equation can be solved as
$$
\vec a_3\
=\ {(\vec a_1\times \vec a_2)^*+c_1\vec a_1+c_2\vec a_2\over
	\Im[\vec a_1^*\cdot\vec a_2]}
\eqn\AThree
$$
for some real coefficients $c_1$ and $c_2$ whose explicit values follow from the
consistency of eq.~\AThree\ with the eqs.~\Derivatives:
$$
c_1\ =\ -\Re(J),\quad c_2\ =\ +\Im(J),\qquad
{\rm where}\quad
J\ =\ \partial_1 z_1\,\partial_2 z_2\ -\ \partial_1 z_2\,\partial_2 z_1\,.
\eqn\Jeq
$$
Re-phrasing eq.~\AThree\ as a differential equation for the independent
coordinates $z_{1,2}(X)$ of a BPS domain wall, we arrive at
$$
\eqalign{
F\,\partial_3\,z_1\ &
=\ (c_1\partial_1+c_2\partial_2)\,z_1\ -\ (i\partial_1+\partial_2)\,z_2^*\,,\cr
F\,\partial_3\,z_2\ &
=\ (c_1\partial_1+c_2\partial_2)\,z_2\ +\ (i\partial_1+\partial_2)\,z_1^*\,,\cr
}\eqn\EQ
$$
where $c_1$ and $c_2$ are as in eq.~\Jeq\ and
$$
F\ \equiv\ \Im[\vec a_1^*\cdot\vec a_2]\
=\ 1\ +\ \Im[\partial_1 z_1^*\,\partial_2 z_1\,+\,\partial_1 z_2^*\,\partial_2 z_2] .
\eqn\Feq
$$

Note that eqs.\EQ\ {\sl disallow} holomorphic embedding of any
fixed--$x_3$--slices $\Sigma(x_3)$ of the BPS domain wall --- except asymptotically
for $x_3\to\pm\infty$ where $\Sigma(x_3)$ asymptotes to holomorphic 2--cycles
$\Sigma_{1,2}$.
Indeed, suppose there were a holomorphic slice in which $z_1$ and $z_2$ are
holomorphic functions of the $z_3=X_1+iX_2$.
In that case, eq.~\Jeq\ would yield $c_1=c_2=0$ while at the same time
$(i\partial_1+\partial_2)z_{1,2}^*=0$; consequently, eqs.~\EQ\ would immediately
result in $\partial_3 z_1=\partial_3 z_2=0$.
And since eqs.~\EQ\ are first-order differential equations with respect to the
$\partial_3$, that would actually mean complete $X_3=x_3$ independence of the
$z_1$ and $z_2$ --- and the solution would be an $x$--independent vacuum, not
a domain wall.

Conversely, a constant vacuum solution should have holomorphically embedded
slices $\Sigma(x_3)\equiv\Sigma$.
Ultimately, this is related to four rather than two supercharges being unbroken,
but we can also see how this degenerate case works in context of the $\vec R=0$
equation:
For the $x_3$--independent $z_1$ and $z_2$, the $\vec R$
reduces to $\vec a_1\times\vec a_2$, so $\vec R=0$ implies $\vec a_1\propto a_2$;
consequently $\vec a_2=i\vec a_1$
(\cf\ eqs.~\Derivatives) \ie, $\partial_2\vec z=i\partial_1\vec z$
and hence $\vec z=\vec z(X_1+iX_2)$ ---  a holomorphic embedding.


Now consider the supersymmetric vacua $\Sigma_{1,2}$ that serve as boundaries of the
BPS wall's 3--cycle $\SS$ --- and hence as boundary conditions for the
equations~\EQ.
For the scalar-less $\NS=1$ SSYM theory, the $\N$ vacua \val\GCondensate\
correspond to Riemann surfaces
$$
z_1^{\N}\ =\ e^{-z_3},\qquad z_2^{\N}\ =\ e^{+z_3},\qquad
z_1 z_2\ =\ S_n,\quad n=1,\ldots,\N
\eqn\Surfaces
$$
where $S_n=e^{2\pi in/\N}$ is precisely the gaugino condensate in $\Lambda_1^3$ units.
\refmark{\WittenQCD,\biksy}
Note that the $z_3$ coordinate is periodic modulo $2\pi i$, so eq.~\Surfaces\
describes exactly $\N$ Riemann surfaces distinguishable by the $Z_{\N}$ phase of
the gaugino condensate.
Moreover,
each of these surfaces $\Sigma_n$ is invariant under a global $U(1)$
symmetry
$$
z_1\ \mapsto\ e^{i\delta}\,z_1\,,\qquad
z_2\ \mapsto\ e^{-i\delta}\,z_2\,,\qquad
z_3\ \mapsto\ z_3\ +\ i\N \delta.
\eqn\Uone
$$
As argued by Witten,\refmark{\WittenQCD}
this exact symmetry of MQCD is completely invisible in the ordinary Supersymmetric QCD,
and hence cannot be spontaneously broken by a domain wall solution:
Indeed, any such breaking would result in some kind of a wall-bound Goldstone mode,
which would not make any sense at all from the ordinary S-QCD point of view.
Therefore, the entire domain-wall's 3--cycle $\SS$ has to be invariant under the
symmetry~\Uone, which allows us to introduce the following ansatz:
$$
\eqalign{
z_1(X)\ &=\ P(X_1,X_3)\,e^{iX_2/\N} ,\cr
z_2(X)\ &=\ Q(X_1,X_3)\,e^{-iX_2/\N} ,\cr
z_3(X)\ &=\ X_1\ +\ iX_2 \cr
}\eqn\WallAnsatz
$$
for some complex functions $P(X_1,X_3)$ and $Q(X_1,X_3)$.
In terms of these functions, eqs.~\EQ\ become
$$
\eqalign{
F\,\partial_3 P\ &
=\ \left(c_1\partial_1\,+\,\coeff{i}{\N}\,c_2\right)\,P\
	-\ i\left(\partial_1+\coeff1\N \right)\,Q^*,\cr
F\,\partial_3 Q\ &
=\ \left(c_1\partial_1\,-\,\coeff{i}{\N}\,c_2\right)\,Q\
	+\ i\left(\partial_1-\coeff1\N \right)\,P^*,\cr
}\eqn\EQPQ
$$
where
$$
J\ =\ \coeff{-i}{\N}\,\partial_1(PQ)\qquad
{\rm and}\quad F\ =\ 1\ +\ \coeff{1}{2\N}\,\partial_1(|P|^2-|Q|^2)
\eqn\JF
$$
while the boundary conditions are simply
$$
\eqalign{
P\ =\ e^{X_1/\N},\quad Q\ =\ S_1\,e^{-X_1/\N} &\qquad {\rm for}\quad X_3\to-\infty,\cr
P\ =\ e^{X_1/\N},\quad Q\ =\ S_2\,e^{-X_1/\N} &\qquad {\rm for}\quad X_3\to+\infty.\cr
}\eqn\BoundaryConditions
$$

Unfortunately, eqs.~\EQPQ\ do not have any non-trivial solutions for which
$S(X)\equiv z_1z_2=PQ$ is a function of the $X_3$ but not of the $X_1$;
we prove this sad theorem in the Appendix~B.
Thus, the domain wall of the MQCD cannot be interpreted in terms of the
$x_3$--dependent gaugino condensate $S(X_3)$.
Of course, even for the SSYM theory we could not explain the BPS domain wall
in terms of the gaugino condensate alone or calculate the actual profile
of the $S(x_3)$, but this was basically a calculational difficulty.
In case of the MQCD, the gaugino condensate profile is not even definable,
let alone computable even in principle.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{MQCD for the $SU(2)$ and the Monge-Ampere Equation.}
\line{\hfil$*$\quad$*$\quad$*$\hfil}

For $\N>2$, the boundary conditions~\BoundaryConditions\ require $P$ and $Q$
to be inherently complex functions of the $X_1$ and the $X_3$, but in the $SU(2)$ case
both the boundary conditions and the equations \EQPQ\ allow for real or purely
imaginary $P$ and $Q$.
Clearly, this is the MQCD counterpart of having real $S(x_3)$ and $U(x_3)$ for the
$SU(2)$ SSYM theory, so let us see how the
MQCD equations simplify for the real solutions;
specifically, let us assume real $P$ and purely imaginary $Q$.
It turns out that in this case, eqs.~\EQPQ\ take a simplified form in terms of
new real variables $S=-iPQ$ and $R=\half(P^2+Q^2)$:
$$
\eqalign{
\partial_3 R\ &
=\ -\partial_1 S,\cr
\bigl(1+\half\partial_1 R\bigr)\,\partial_3 S\ &
=\ -\half(\partial_1 S)^2\ +\ \partial_1 R\ \pm\sqrt{S^2+R^2}\,,\cr
}\eqn\EQSR
$$
while the boundary conditions read
$$
S(X_3\to\mp\infty)\ \to\ \pm1,\qquad
R(X_3\to\mp\infty)\ \to\ \sinh(X_1).
\eqn\BouCondSR
$$

The first equation~\EQSR\ allows us to introduce a single variable $\psi(X_1,X_3)$
such that $S=\partial_3\psi$ and $R=-\partial_1\Psi$.
Substituting this into the second eq.~\EQSR\ gives us a  {\sl Monge--Ampere} equation
$$
\half\left[(\partial_1\partial_3\Psi)^2\,-\,(\partial_1^2\Psi)(\partial_3^2\Psi)\right]
=\ \nabla^2\psi\ \pm\sqrt{(\nabla\psi)^2}
\eqn\MonAmp
$$
subject to the boundary conditions
$$
\psi(X_3\to\mp\infty)\ =\ \pm X_3\ -\ \cosh(X_1).
\eqn\BoundCondPsi
$$
This reduction to a single --- but fourth order --- Monge--Ampere equation was first
noticed by A.~Volovich.\refmark\Volovich 
She has also constructed a formal solution as an infinite power series in $(1/\cosh^2X_3)$;
unfortunately, the series diverges, so it is not clear whether her solution actually
exists.

The Monge--Ampere equations have been extensively studied by mathematicians
\refmark\MAbook\
and for many equations of this type, the existence of a unique solution
is guaranteed by a theorem.
Unfortunately, such theorems do not apply to the specific Monge--Ampere eq.~\MonAmp,
so at present we do not have a rigorous existence proof for a BPS-saturated domain wall
in MQCD.
Clearly, more research in this direction would be very helpful.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%(3) Monge Ampere cannot reproduce a wall of width of  ${1\over \Lambda}$  
%
%(4) The equation does not contain information on $\Lambda$ only the 
%boundary contions.
%
%(5) scalling argument scale $\psi\rightarrow \lambda \psi$
%and $\pa\rightarrow \gamma\pa$ then one can classify the various
%terms of the Monge-Ampre equation and wth that get various 
%approximated equations.  
%
%(6) Solution with 
%$\psi(\rho) S={Kx_1e^{\pm\rho}\over \rho^2}$ where  $\rho=
%\sqrt{x_1^2+x_3^2}$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\line{\hfil$*$\quad$*$\quad$*$\hfil}

Finally, consider the MQCD corresponding to the supersymmetric gauge theory with an
adjoint scalar $\Phi$.
In the $SU(2)$ case, the Riemann surfaces $\Sigma$ of supersymmetric vacua have genus
$g=0$ and general analytic form
$$
e^{2z_3}\ +\ 2e^{z_3}(z_1^2-U)\ +\ \Lambda_2^4\ =\ 0,\qquad
z_2^2\ -\ m^2z_1^2\ -\ 2mS\ =\ 0\,;
\eqn\MVYTVacua
$$
the $g=0$ requirement allows for just two such surfaces, with parameters $U$ and $S$
precisely as in eqs.~\TwoVYTVacua\ for the vacua of the gauge theory,
and it is these two surfaces 
$$
\eqalign{
\Sigma_1\,:\quad&
z_1z_2\ =\ m\left( z_1^2-e^{z_3}+\Lambda_2^2\right),\quad
    z_2^2\ =\ m^2\left(z_1^2-2\Lambda_2^2\right),\cr
\Sigma_2\,:\quad&
z_1z_2\ =\ m\left( z_1^2-e^{z_3}-\Lambda_2^2\right),\quad
    z_2^2\ =\ m^2\left(z_1^2+2\Lambda_2^2\right) \cr
}\eqn\MVYTSurfaces
$$
that serve as boundaries of the supersymmetric 3--cycle $\SS$ describing the BPS
domain wall.

We are particularly interested in the MQCD analogue of the Seiberg--Witten domain wall
in the small $m$ limit --- where all fields change but slowly with the $x_3$
and the physics inside the wall is in the Coulomb phase of the massless SW theory.
By analogy, we expect approximately holomorphic slices $\Sigma(x_3)$, slowly changing
with the $x_3$ and also $|z_2|\ll|z_1|$ (in the massless limit, $z_2\mapsto 0$).
Let us therefore assume holomorphic dependence of the $z_1$ coordinate on the
$X_1+iX_2=z_3$ but allow for a non-holomorphic $z_2(z_3,\bar z_3,X_3)$.

In terms of the world-volume coordinates $z_3$, $\bar z_3$ and $x_3$ and the
corresponding derivatives $\partial=\half\bigl(\partder{}{X_1}-i\partder{}{X_2}\bigr)$,
$\bar\partial=\half\bigl(\partder{}{X_1}+i\partder{}{X_2}\bigr)$
and $\nabla=\partder{}{x_3}$, eqs.~\EQ\
become
$$
\eqalign{
F\nabla z_1\ & =\ - J^*\partial z_1\ -\ J\bar\partial z_1\ -\ 2i\partial z_2^*,\cr
F\nabla z_2\ & =\ - J^*\partial z_2\ -\ J\bar\partial z_2\ +\ 2i\partial z_1^*,\cr
}\eqn\EQhol
$$
where
$$
\eqalign{
F\ &=\ 1\ +\ |\partial z_1|^2\ -\ |\bar\partial z_1|^2\
	 +\ |\partial z_2|^2\ -\ |\bar\partial z_2|^2,\cr
J\ &=\ 2i(\bar\partial z_1\,\partial z_2\ -\ \bar\partial z_2\,\partial z_1).\cr
}\eqn\FJhol
$$
In the holomorphic $z_1$ approximation,
$F\approx1+|\partial z_1|^2$ (since $|z_2|\ll|z_1|$), $J=-2i\bar\partial z_2\partial z_1$
and the eqs.~\EQhol\ simplify to
$$
\eqalign{
\nabla z_1\ &
=\ -2i\partial z_2^*,\cr
\nabla z_2\ &
=\ {2i\over F}\,\left(\partial z_1(\bar\partial z_2)^2\
	-\ \bar\partial z_1^*\,\partial z_2^*\,\partial z_2\right) .\cr
}\eqn\EQsimp
$$
Note that the first equation here implies $\bar\partial\partial z_2^*=0$
and hence
$$
z_2(z_3,\bar z_3,x_3)\ =\ f(z_3,x_3)\ +\ g^*(\bar z_3,x_3)
\eqn\Ztwo
$$
where $f$ and $g$ are holomorphic functions of the $z_3$.
The boundary conditions for these functions (and also the $z_1(z_3,x_3)$ are
$$
\vcenter{\openup 2\jot
\ialign{$\displaystyle{#}\,$,\quad\hfil& $\displaystyle{#}\,$,\quad\hfil&
	$\displaystyle{#}$\quad\hfil& #\hfil\cr   
    z_1\,\to\,\tilde\Lambda\,\cosh{\tilde z_3\over2}&
    f\,\to\,m\tilde\Lambda\,\sinh{\tilde z_3\over2}&
    g\,\to\,0 & for $x_3\to -\infty$,\cr
    z_1\,\to\,\tilde\Lambda\,\sinh{\tilde z_3\over2}&
    f\,\to\,m\tilde\Lambda\,\cosh{\tilde z_3\over2}&
    g\,\to\,0 & for $x_3\to +\infty$,\cr
}}\eqn\BoundCondZFG
$$
where $\tilde\Lambda=i\sqrt{2}\Lambda_2$ and $\tilde z_3=z_3-\log\Lambda_2^2$.

The second eq.~\EQsimp\ can be further simplified by assuming either
$|\partial z_1|^2\gg1$ or $|\partial z_1|^2\ll1$ in units of the eq.~\MVYTVacua.
These assumptions give us respectively $F\approx|\partial z_1|^2$ or $F\approx1$,
and in both cases holomorphy of the $f$ and $g$ functions can be used to derive
separate equations for the $\nabla f$ and $\nabla g$.
Alas, in both cases the resulting equations are inconsistent with the boundary
conditions~\BoundCondZFG,
which means that the BPS domain wall in MQCD defies simplification.
At best, $|\partial z_1|^2$ cannot be either large or small throughout
the supersymmetric 3--cycle~$\SS$, but it is also possible that the
holomorphy approximation $\bar\partial z_1\approx0$ has to break down
in some part of the 3--cycle's world-volume.




\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Eqs.~\EQsimp\ can be further simplified by assuming either $|\partial z_1|^2\gg1$
or $|\partial z_1|^2\ll1$ in units of the eq.~\MVYTVacua.
For $|\partial z_1|^2\gg1$ we have $F\approx|\partial z_1|^2$,
which lets us reorganize eqs.~\EQsimp\
into three equations for three $x_3$--dependent holomorphic functions of the $z_3$,
namely
$$
\nabla f\ =\ -2i\,{(\partial f)(\partial g)\over\partial z_1}\,,\qquad
\nabla g\ =\ -2i\,{(\partial g)^2\over\partial z_1}\,,\qquad
\nabla z_1\ =\ -2i\partial g.
\eqn\ThreeEqs
$$
This equation system has a general solution of the form
$$
f(z_3,x_3)\ =\ f(z_1(z_3,x_3)),\quad
g(z_3,x_3)\ =\ g(z_1(z_3,x_3));
\eqno\eq
$$
Unfortunately, this general solution is incompatible with the boundary
conditions~\BoundCondZFG.

In the opposite $|\partial z_1|^2\ll1$ regime $F\approx1$,
which makes for a different holomorphy structure
of the right hand side of the second eq.~\EQsimp.
Consistency of this structure with the $\nabla(f+g^*)$ on the left hand side of the
equation imposes severe constraints on the $f$, $g$ and $z_1$ functions;
after a bit of tedious algebra, these constraints lead to linear equations
$$
\nabla f\ =\ A(x_3)\,\partial z_1,\qquad
\nabla g\ =\ B(x_3)\,\partial z_1,\qquad
\nabla z_1\ =\ -2i\partial g
\eqn\EQlinear
$$
for some $z_3$--independent $A(x_3)$ and $B(x_3)$.
In light of the boundary conditions~\BoundCondZFG, the solutions should have
general form
$$
\eqalign{
z_1\ &=\ \chi(x_3)\cosh{z_3\over2}\ +\ \varphi(x_3)\sinh{z_3\over2}\,,\cr
g\ &=\ i\varphi'(x_3)\cosh{z_3\over2}\ +\ i\chi'(x_3)\sinh{z_3\over2}\,,\cr
f\ &=\ \xi(x_3)\cosh{z_3\over2}\ +\ \eta(x_3)\sinh{z_3\over2}\,,\cr
}\eqn\GenSolution
$$
where the functions $\chi(x_3)$, $\varphi(x_3)$, $\xi(x_3)$ and $\eta(x_3)$
should satisfy the following constraints:
$$
\vcenter{\ialign{$\displaystyle{#}$\quad\hfil\cr
\chi''\varphi\ =\ \varphi''\chi,\qquad
    \xi'\chi\ =\ \eta'\varphi,\cr
{\rm for}\ x_3\to-\infty,\quad
	\chi\to\tilde\Lambda,\ \varphi\to0,\ \xi\to0,\ \eta\to m\tilde\Lambda,\cr
{\rm for}\ x_3\to+\infty,\quad
	\varphi\to\tilde\Lambda,\ \chi\to0,\ \eta\to0,\ \xi\to m\tilde\Lambda.\cr
}}\eqn\Constraints
$$
Unfortunately, these constraints are inconsistent too.
Alas, the BPS domain wall of MQCD defies simplification!

\endinput
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> Master.tex <==
%auto-ignore
%% Master TeX file for the DomainWall paper
% 
\let\flatsourcedir=Y	% Flat directory tree
\let\sizeselector=U	% UN-reduced output
\let\makehyperlinks=Y	% YES
\input macros.tex
\chapterinput Titlepage.tex
\chapterinput Biblio.tex
\chapterinput Intro.tex
\chapterinput SWsummary.tex
\chapterinput ToyModel.tex
\chapterinput SWwall.tex
\chapterinput SWlimits.tex
\chapterinput GauginoCond.tex
\chapterinput MQCD.tex
\chapterinput Summary.tex
\chapterinput Appendices.tex
\refout
\bye



==> NoHyper.tex <==
%&tex
%% Master TeX file for the DomainWall paper
% 
\let\flatsourcedir=Y	% Flat directory tree
\let\sizeselector=U	% UN-reduced output
\let\makehyperlinks=N	% NO
\input macros.tex
\chapterinput Titlepage.tex
\chapterinput Biblio.tex
\chapterinput Intro.tex
\chapterinput SWsummary.tex
\chapterinput ToyModel.tex
\chapterinput SWwall.tex
\chapterinput SWlimits.tex
\chapterinput GauginoCond.tex
\chapterinput MQCD.tex
\chapterinput Summary.tex
\chapterinput Appendices.tex
\refout
\bye



==> README <==
%auto-ignore
This the README file for the distributed TEX source of the Domain Wall paper
by VK, JS and SY.  There is a lot of files in this source, hence this README
file to help you find your way.

To TeX the paper, simply
	tex Master.tex
and it should input all the other files.  If you use GUI version of TeX
(ie., on a Macintosh), make sure to use plain TeX and not LaTeX.

To save paper, you may want to print the paper in two-pages-on-one-sheet
format.  To do that, simply
	tex Reduced.tex
instead of TeXing the Master.tex file.

Finally, if your DVI->printer system or DVI previewer has problems with
the hyperlinks imbedded into the DVI file,
	tex NoHyper.tex
instead of Master.tex.

All the other files in the source are automatically input by the Master.tex
or its Reduced.tex and NoHyper.tex equivalents.  You do not really need to
know what they are and what they do, but if you are curious, here is a brief
description:  Files 
	Titlepage.tex
	Intro.tex
	SWsummary.tex
	ToyModel.tex
	SWwall.tex
	SWlimits.tex
	GauginoCond.tex
	MQCD.tex
	Summary.tex
	Appendices.tex
	Biblio.tex
contain the appropriate sections of the paper.  Files
	f1.tex  f2.tex  f3.tex  f4.tex  f5.tex  f6.tex  f7.tex  f8.tex
contain the figures.  Figure 7 uses EPS graphics, hence f7.eps file.
All the other figures use PiCTeX; the curves are saved in \replot format
in 21 *.saved files
	f1a-D.saved     f1b-T.saved     f3a-gth.saved   f5-M.saved
	f1a-M.saved     f2-D.saved      f3b-U.saved     f5-U.saved
	f1a-T.saved     f2-M.saved      f4-M.saved      f6-S.saved
	f1b-D.saved     f2-T.saved      f4-U.saved      f8-S1.saved
	f1b-M.saved     f3a-g.saved     f5-D.saved      f8-S2.saved
							f8-S3.saved
Finally, there are macro files
	macros.tex
	phyzzx.tex
	epsf.tex
	pictex.tex
	hyperbasics.tex
The macros.tex file is made for this paper only. Files epsf.tex, pictex.tex,
phyzzx.tex and hyperbasics.tex are standard; they are included with the source
to insure that you have the right version.


==> Reduced.tex <==
%auto-ignore
%% Master TeX file for the DomainWall paper
% 
\let\flatsourcedir=Y	% Flat directory tree
\let\sizeselector=R	% Reduced output
\let\makehyperlinks=Y	% YES
\input macros.tex
\chapterinput Titlepage.tex
\chapterinput Biblio.tex
\chapterinput Intro.tex
\chapterinput SWsummary.tex
\chapterinput ToyModel.tex
\chapterinput SWwall.tex
\chapterinput SWlimits.tex
\chapterinput GauginoCond.tex
\chapterinput MQCD.tex
\chapterinput Summary.tex
\chapterinput Appendices.tex
\refout
\bye



==> SWlimits.tex <==
%auto-ignore
%
% Section 5 of the DomainWall paper
%
\chapter{Limitations of the Seiberg--Witten Theory}
%
Beyond the very-small-mass limit~\SWRatioLimit,
the two transitional regions of the SW domain wall not only take over
the entire wall's thickness but also overlap each other.
Consequently, {\sl the monopole and the dyon condensates now coexist in the
same region of space}.
In the toy model with $h\gsim\Lambda$, similar coexistence of the $\vev\mono$
and $\vev\dyon$ condensates was a mere calculational inconvenience since
both the `monopoles' and the `dyons' were actually electrically charged
fields of the same local field theory.
In the Seiberg--Witten case however, we have a real problem:
The monopoles and the dyons are now true to their names and thus cannot be
simultaneously described as local fields; consequently, {\sl we simply
do not have a theory to describe coexisting condensates $\vev\mono$
and $\vev\dyon$.}

Naturally, before we bust our brains trying to develop such a theory,
we would like to know whether it would actually solve the problem at hand.
Specifically, the question is whether an effective theory somehow comprising five
chiral multiplets $\mono$, $\amono$, $\dyon$, $\adyon$ and $U$ would be able to
adequately describe the SW domain wall for $m\gsim O(\Lambda)$?
The answer to this question turns out to be negative:
The overlapping monopole and dyon condensates are only a part of our problem
as the entire Seiberg--Witten theory reaches the limit of its validity.

The basic limitation of the Seiberg--Witten theory is that it's basically the effective
low-energy --- \ie, long-distance --- theory of the massless fields, namely
the $U$ modulus and its $\NS=2$ superpartners.
It gives us the exact two-derivative interactions of those fields (encoded
in the $U$ dependent gauge coupling~\SWGaugeCoupling\ and metric~\SWMetric),
but it tells us nothing about the four-derivative, six-derivative,
\etc, interactions because they are not protected by the $\NS=2$ supersymmetry.
Such higher-derivative interactions are literally irrelevant to the long-distance
limit of the theory, but they are very much relevant to the finite-size
field configurations such as finite-thickness domain walls.

Indeed, consider a BPS-saturated domain wall in a generic $\NS=1$ effective
field theory.
The exact BPS equations
$$
V^\mu_a(x_3)\ =\ 0,\qquad D_a(x_3)\ =\ 0,\qquad
{d A^i\over dx_3}\ =\ e^{i\varphi}\,F^i
\eqn\BPSGeneric
$$
follow from eq.~\PreservedQ, but they
are of little practical use without specific formul\ae\ for the auxiliary fields
$D_a$ and $F^i$ in terms of the physical scalar fields $A^i$.
Such formul\ae\ follow from the generating functional $\Gamma$ (also known as `the
effective classical Lagrangian') of the effective theory.
Truncating $\Gamma$ to terms with four or less
super-derivatives (\ie, two derivatives or four fermions or two $F$'s) results in
$F^i=g^{i\bar\jmath}W^*_{\bar\jmath}$ and hence eqs.~\BPSWall\
for the domain wall, but allowing for higher-derivative terms
would make for much more complicated formul\ae.
In particular, at the six-super-derivative level one has quadratic equations
for the auxiliary fields $F^i$ while at still higher derivative level the $F^i$
become propagating fields governed by differential (rather than merely polynomial)
equations.
%\Vnote{Do we need to explain this or is there a reference?}
Examples of such equations are presented in Appendix~A but their
specific form is not germane to the present discussion;
it suffices to say that they are quite complicated.
Consequently, the exact equations for the BPS domain walls' profiles depend
in a complicated way on the higher-derivative terms in the effective Lagrangian
$\Gamma$.
Generally, one needs to know all the terms in $\Gamma$ that are important
at the distance scale of the wall's thickness:
For the thick walls, only the superpotential, the K\"ahler function and the gauge
couplings are important and the wall's profile can be described
by the approximate eqs.~\BPSWall;
the thin walls are much more complicated.

The Seiberg--Witten theory is the infrared limit of the $\NS=2$ SSYM theory;
it is valid at distances $\ell>1/\Lambda$ but breaks down at shorter
distances.
Indeed, the SSYM theory has various ``hadrons'' with masses $O(\Lambda)$
--- not just the
monopoles $\mono,\amono$ and the dyons $\dyon,\adyon$, but many other BPS
saturated and unsaturated particles as well.
Once all those hadrons are integrated out of the effective low-energy theory,
the resulting effective SW Lagrangian $\Gamma$ acquires
all kinds of higher-derivative terms, which are irrelevant in the very long
distance limit but become very important at $\ell\lsim O(1/\Lambda)$.
Consequently, we may use the long-distance
 SW theory to describe domain walls that happen to be much thicker
than $O(1/\Lambda)$ --- and the thicker the wall, the more accurate the description
--- but the thinner walls are governed by the shorter-distance theory and
cannot be adequately described in the SW terms.
The wall's thickness (in $1/\Lambda$ units) decreases with
the $\NS=2$ breaking mass parameter $m$.
Thus, {\sl for small $m/\Lambda$ ratios, the domain wall is thick and
the field profiles inside it are governed by the Seiberg--Witten theory;
but for large $m/\Lambda$, the domain wall is thin and the SW theory
simply does not apply.}

\endinput


==> SWsummary.tex <==
%auto-ignore
%
% Section 2 of the DomainWall paper
%
\chapter{Overview of Seiberg--Witten Theory}
%
The strongest evidence for the vacuum structure of the $\NS=1$ SSYM
theories comes from the Seiberg--Witten (SW) theory 
of the $\NS=2$ SSYM.\refmark\sw\
A non-abelian gauge theory with unbroken $\NS=2$ supersymmetry and
without any `quark' hypermultiplets
has a continuous family of exactly degenerate vacua.
The {\sl moduli space} of these vacua has a complex dimension
equal to the rank $r$ of the gauge group.
For a generic vacuum, the theory is in the abelian Coulomb phase:
The gauge group $G$ is spontaneously broken down to its maximal abelian
subgroup $U(1)^r$ and the only massless particles
are the $r$ gauge bosons and their $\NS=2$ superpartners.
However, the moduli space has singular subspaces where some charged
hypermultiplets of particles are also massless.

For the sake of simplicity, we focus this article on
the $SU(2)$ SSYM theory where the vacuum
expectation value $U=\vev{\tr\Phi^2}$\foot{%
	The $\Phi$ here is the adjoint multiplet of the gauge
	symmetry comprised of the scalar $\NS=2$ superpartners
	of the gauge fields; the trace is taken in the fundamental
	representation.
	}
serves as a global complex coordinate of the one-dimensional moduli space
of the theory.
Thanks to the $\NS=2$ supersymmetry, the K\"ahler metric for the
$U$ field is known exactly as
$$
g_{U\overline U}(U)\ =\ {1\over 4\pi}\,\Im\left(
	\partder{A_2}{U}\,\partder{A_1^*}{U^*}\right) ,
\eqn\SWMetric
$$
where $A_1(U)$ and $A_2(U)$ are the two periods of the Seiberg--Witten
elliptic curve,
$$
A_{1,2}(U)\ =\ {\sqrt{2}\over2\pi}\!
\oint_{\rm contour_{1,2}} {(x-U)\,dx\over\sqrt{x^3-2Ux^2+\Lambda^4x}}\,.
\eqn\EllipticCurve
$$
The $U$-dependence of the abelian gauge coupling is given by
$$
{2\pi i\over g^2}\ +\ {\Theta\over 4\pi}\ \equiv\ \tau\
=\ {dA_2(U)\over dA_1(U)}\,;
\eqn\SWGaugeCoupling
$$
this analytic function has non-trivial monodromies around its singularities;
physically, the monodromies amount to electric-magnetic duality transformations,
$$
\tau\,\to\,{a\tau+b\over c\tau+d}\,,\qquad
({\bf E}-i{\bf B})\,\to\,(c\tau+d)\,({\bf E}-i{\bf B}) .
\eqn\SWDUality
$$
In duality-invariant terms, the $U$-dependence of the gauge coupling
can be summarized as
$$
j(\tau)\ =\ {(16U^2-12\Lambda^2)^3\over\Lambda^8(U^2-\Lambda^4)}\,.
\eqn\SWj
$$

At two points in the moduli scape, namely at $U=\pm\Lambda^2$,
a magnetically charged hypermultiplet becomes massless
and the gauge coupling \SWGaugeCoupling\ and the K\"ahler metric \SWMetric\
have logarithmic singularities;
mathematically, this corresponds to degeneration of the SW elliptic curve.
The hypermultiplet $\mono$ which becomes massless at $U=+\Lambda^2$
is a magnetic monopole without electric charge, $(q_e=0,q_m=1)$,
while at $U=-\Lambda^2$, the massless hypermultiplet is a dyon with
charges $(q_e=1,q_m=1)$.
For $U$ being close to either singularity, the low-energy
regime of the SW theory is described by a {\sl local} effective
field theory, namely $\NS=2$ SQED with one ``electron'' ---
which is actually $\mono$ or $\dyon$ whose charge is rendered purely
electric by means of a
suitable electric-magnetic duality transformation.

{}From the $\NS=1$ point of view, the $\NS=2$ SSYM theory is a gauge
theory with a chiral supermultiplet $\Phi$ in the adjoint representation
of the gauge group,
and the second supersymmetry can be softly broken by giving $\Phi$
a non-zero mass.
When this happens to the Seiberg--Witten theory,
the mass term $m\tr(\Phi^2)$ for the $SU(2)$ triplet $\Phi$ in the
superpotential
becomes the O'Raighfeartaigh F-term\refmark\Oraigh\  $mU$ for
the $U$ modulus (viewed now as an $\NS=1$ chiral superfield).
Consequently, the energy density of a generic $\NS=2$ SW vacuum
(where $mU$ comprises the entire superpotential of the
effective low-energy theory)
is lifted to ${|m|^2g^{U\overline U}>0}$.

On the other hand, the singular vacua with $U=\pm\Lambda^2$
remain $\NS=1$ supersymmetric vacua: Instead of breaking SUSY,
the O'Raighfeartaigh term now causes confinement.
%
Indeed, at the $U=+\Lambda^2$ singularity, the superpotential of
the effective low-energy theory is
$$
\eqalign{
W\ &=\ mU\ +\ A_2(U)\,\mono\amono\cr
&\approx\ mU\ +\ {\Lambda^2-U\over i\sqrt{2}\Lambda}\,\mono\amono\cr
}\eqn\SWMagneticW
$$
where $\mono$ and $\amono$ are the chiral monopole/antimonopole
superfields.
This superpotential --- together with the $U(1)$ gauge superfield
magnetically dual to the electric $U(1)\subset SU(2)$ ---
has a unique supersymmetric vacuum
$$
U\ =\ +\Lambda^2,\qquad
\mono\amono\ =\ i\sqrt{2}\Lambda m,\qquad
|\mono|\ =\ |\amono|.
\eqn\SWConfiningVacuum
$$
{}From the dual $U(1)$ point of view, the fields $\mono$ and $\amono$
are electrically charged and their non-zero vacuum expectation values
imply electric superconductivity {\it \`a~la}~Higgs;
the photon becomes massive and the magnetic charges suffer confinement.
However, as far as the original $U(1)\subset SU(2)$ gauge theory
is concerned, the superconductivity is magnetic
and the confined charges are electric;
this is the familiar {\sl electric confinement} of a non-abelian
gauge theory.

Likewise, at the other singularity $U=-\Lambda^2$, the effective
superpotential is
$$
\eqalign{
W\ &=\ mU\ +\ \left(A_1(U)+A_2(U)\right)\,\dyon\adyon\cr
&\approx\ mU\ +\ {\Lambda^2+U\over -i\sqrt{2}\Lambda}\,\dyon\adyon\cr
}\eqn\SWDyonicW
$$
and the vacuum
$$
U\ =\ -\Lambda^2,\qquad
\dyon\adyon\ =\ i\sqrt{2}\Lambda m,\qquad
|\dyon|\ =\ |\adyon|
\eqn\SWObliqueVacuum
$$
is a dyonic superconductor which confines particles with charges
$q_e\neq q_m$;
such behavior is called {\sl oblique confinement}.

To summarize the phase structure of the Seiberg--Witten theory,
the theory with $m=0$ and unbroken $\NS=2$ SUSY is in the abelian
Coulomb phase with a moduli space while the $\NS=1$ theory with $m\neq0$
has an electric confinement phase and an oblique confinement phase,
each comprising an isolated vacuum without any massless particles at all.
When $m$ becomes large compared to $\Lambda$, eqs.~\SWConfiningVacuum\
and \SWObliqueVacuum\ for the monopole/dyon expectation values
should be renormalized to account for
quantum corrections to the K\"ahler metric for those fields,
but the two confining phases persist all the way to $m\to\infty$ limit
when the $\Phi$ superfield decouples and the SW theory reduces to
$\NS=1$ SSYM; this point is discussed in more detail in section~6.

Note that the phase structure of the $\NS=1$ SW theory follows from
three separate low-energy effective {\sl local} field theories
covering different parts of the $\NS=2$ moduli space,
namely the generic $U$ away from the singularities,
the singular region of $U\approx+\Lambda^2$ and
the other singular region of $U\approx-\Lambda^2$.
The Seiberg--Witten analysis has no need for a single effective theory
covering the entire moduli space --- which is very fortunate since
such a theory does not exist, at least not as a local field theory.
Indeed, such a theory would have to include both $\mono,\amono$
and $\dyon,\adyon$ as local fields, both locally coupled to the
same $U(1)$ gauge field $V_\mu$, which would require them to have
purely-electric charges {\sl in the same duality frame},
a mathematical impossibility.

Unfortunately, a domain wall between the two confining vacua
--- the main subject of this article ---
has the modulus field continuously changing its value from $U\approx+\Lambda^2$
on one side of the wall through generic values of $U$ in the middle
all the way to $U\approx-\Lambda^2$ on the other side; thus one
has to use three different effective theories in different regions
of space to understand the whole wall.
Worse, {\sl the field configuration in the middle of the wall
is not a vacuum}, so the effective theory for a generic $\NS=2$ SW vacuum
is of questionable validity for this region, --- and we do not have
a better theory to replace it with.

We shall see momentarily
that the answer to the last question depends on
the $m/\Lambda$ ratio: For small $m\ll\Lambda$, the middle section
of the BPS-saturated domain wall is basically in the adiabatically
perturbed Coulomb phase of the SW theory while the monopole and the
dyon fields become significant only in the two outer sections, ---
and no region of space has both the monopole and the dyon condensates.
Consequently, using all three effective low-energy theories,
 we shall explicitly construct the entire field configuration
of the BPS-saturated domain wall and thus confirm its existence
in a fairly convincing manner.
On the other hand, for large $m\ge O(\Lambda)$, the monopole and the
dyon condensates spread towards each other and presumably overlap,
whatever that means.
Since we see no sign of a phase transition in the theory at finite $m$,
the BPS-saturated domain wall presumably continues to exists all the way
to $m=\infty$ \ie, in the $\NS=1$ SSYM theory,
but the detailed structure of such a wall remains out of our reach.

\endinput


==> SWwall.tex <==
%auto-ignore
%
% Section 4 of the DomainWall paper
%
\chapter{Seiberg--Witten Domain Walls
	 in the $\NS=2$ limit $m\ll\Lambda$}
%
Applying the general conclusions of the previous subsection to the
Seiberg--Witten theory\refmark\sw\ immediately tells us that for {\sl small}
$m$, the SW domain wall has a three-domain structure with the
middle domain occupied by the Coulomb phase adiabatically perturbed
by the O'Raighfeartaigh term $mU$.\refmark\Oraigh\ 
Since $U$ is the only light scalar field in this phase,
the BPS equations~\BPSWall\ reduce to a single equation
$$
{dU\over dx_3}\ = m^*e^{i\varphi} g^{U\overline U}.
\eqn\SWCoulombPhase
$$
Without loss of generality, we assume real positive $m$ and $\Lambda$,
which makes for $e^{i\varphi}=-1$ and real $U(x_3)$ throughout the
Coulomb domain (and indeed the whole domain wall, as we shall see in
a moment).
Eq.~\SWCoulombPhase\ has an obvious formal solution
$$
mx_3\ = \int^0_U\!\!dU'\,g_{U\overline U}(U'),
\eqn\SWFormal
$$
in terms of the K\"ahler metric~\SWMetric.
The latter follows from the
elliptic curve's periods~\EllipticCurve, which in turn
can be expressed in terms of hypergeometric functions.\refmark\KLT\
Unfortunately, the resulting formula
is too complicated to evaluate the integral~\SWFormal\ analytically.
Figure~3a shows the numerical behavior of the metric for real $U$
between $-\Lambda^2$ and $+\Lambda^2$:
It looks rather flat, except for mild logarithmic singularities at the
two ends of the graph; analytically
$$
g_{U\overline U}(U)\ \approx\ {1\over 16\pi^2\Lambda^2}\,
	\log{64\Lambda^4\over\Lambda^4-U^2}
\eqn\SWApproxMetric
$$
for $U\to\pm\Lambda^2$.
\figinsert{f3}
Naively, this logarithmic behavior seems to be limited to $U$ being
fairly close to $\pm\Lambda^2$, but actually, the approximation
\SWApproxMetric\ is amazingly accurate throughout the
$-\Lambda^2$ to $+\Lambda^2$ range: The error is barely 5\% in the
middle of the range (\ie, $U\approx0$) and decreases towards its ends.
At the moment, we  have no explanation for this unexpected accuracy
but only a conjecture that it reflects some important feature of the
dual instanton expansion of the SW theory;
this is a subject for future research.

Substituting the approximate metric~\SWApproxMetric\ into eq.~\SWFormal\
gives us the (approximate) field profile of the Coulomb domain within
the BPS domain wall:
$$
16\pi^2m\,x_3\
=\ \log{\Lambda^2+U\over\Lambda^2-U}\
-\ {U\over\Lambda^2}\,\log{64e^2\Lambda^4\over\Lambda^4-U^2}\,;
\eqn\SWApproxProfile
$$
as expected, the Coulomb domain has finite thickness
$w={1+\log4\over4\pi^2m}\approx0.0605\,m^{-1}$.
For a better accuracy, we have numerically integrated eq.~\SWFormal\
using the exact metric~\SWMetric:
The resulting field profile is presented on figure~3b and the Coulomb
domain's thickness turns out to be $w=0.0625\,m^{-1}$. 

Next, consider the transition regions between the Coulomb and the
confining domains.
According to general rules, the monopole fields $\mono$ and $\amono$
which play a key role in electric-confinement phase are also important
in the transition region between that phase's domain and the Coulomb
domain, but they do not show up in the other regions of the wall.
Likewise, the dyon fields $\dyon$ and $\adyon$ are limited to the
oblique-confinement phase and the transition between that phase
and the Coulomb phase.
Hence, {\sl the monopole and the dyon fields are spatially segregated
from each other} and thus can be taken care of by separate but local
effective field theories.

Because of the obvious symmetry between the two transition regions,
we shall limit our discussion to the electric-confinement-to-Coulomb
transition on the left side of the wall.
The effective field theory governing this transition region has
$\mod$, $\mono$ and $\amono$ fields and the superpotential~\SWMagneticW;
consequently, the BPS equations for this region are
$$
\eqalign{
g_{U\overline U}\,{dU\over dx_3}\ &
=\ -m\ +\ {i\over\sqrt{2}\Lambda}\,\mono^*\amono^* ,\cr
g_\mono\,{d\mono\over dx_3}\ &
=\ {\Lambda^2-U^*\over i\sqrt{2}\Lambda}\,\amono^* ,\cr
g_\mono\,{d\amono\over dx_3}\ &
=\ {\Lambda^2-U^*\over i\sqrt{2}\Lambda}\,\mono^* ,\cr
|\mono|\ & \equiv\ |\amono|,\cr
}\eqn\SWTransitionBPS
$$
where $g_\mono$ is a short-hand notation for the K\"ahler metric
$g_{\mono\overline\mono}=g_{\amono\overline{\amono}}$ for the monopole
fields.
In the $\NS=2$ limit of the SW theory, this metric is $U$-independent
(hypermultiplets' metric does not depend on vector-multiplet moduli)
and can be taken to be canonical, $g_\mono=1$.

The boundary conditions for eqs.~\SWTransitionBPS\ at $x_3=-\infty$
are given by the vacuum expectation values~\SWConfiningVacuum.
Note that both the boundary conditions and the equations~\SWTransitionBPS\
themselves are invariant under complex conjugation of the fields
$U$, $\mono$ and $i\amono$, which means that
the unique BPS-saturated domain wall solution should involve real fields
$U$ and $\mono$ and imaginary $\amono\equiv i\mono$
(modulo a gauge symmetry of the $\mono$ and $\amono$ fields).
Let us therefore substitute
$$
-i\amono\ =\ \mono\ =\ h\,e^{-\alpha/2} ,\qquad
U\ =\ \Lambda^2\ -\ \sqrt{\half}\,\Lambda\beta
\eqn\SWTransitionVars
$$
where $h^2=\sqrt{2}\Lambda m$.
In terms of our new variables $\alpha(x_3)$ and $\beta(x_3)$,
eqs.~\SWTransitionBPS\ become
$$
\eqalign{
{d\alpha\over dx_3}\ & =\ \beta,\cr
{\Lambda g_{U\overline U}(\beta)\over\sqrt{2}}\,{d\beta\over dx_3}\ &
=\ m\left(1-e^{-\alpha}\right) .\cr
}\eqn\SWEoM
$$

Weirdly, this equation system has the form of a classical Hamiltonian or
Lagrangian system where $x_3$ plays the role of time, $\alpha$ is
the canonical position variable, $\beta$ is the velocity,
$$
\rho\ = \int \coeff{\Lambda}{\sqrt{2}}\,
	g_{U\overline U}(\beta)\,d\beta\
\approx\ {\beta\over 16\sqrt{2}\pi^2\Lambda}\,
	\log{32\sqrt{2}e\Lambda\over\beta}
\eqn\SWMomentum
$$
is the canonical momentum conjugate to $\alpha$,
\foot{The approximation in this formula corresponds to
    $g_{U\overline U}\approx(4\pi\Lambda)^{-2}
    \log(32\sqrt{2}\Lambda/\beta)$,\brk
    \cf\ eq.~\SWApproxMetric.}
$$
K\ = \int \beta d\rho\
\approx\ {\beta^2\over 64\sqrt{2}\pi^2\Lambda}\,
	\log{2048e\Lambda^2\over\beta^2}
\eqn\SWKinetic
$$
is the kinetic energy and
$$
V\ =\ -m\left(\alpha-1+e^{-\alpha}\right)
\eqn\SWPotential
$$
is the potential energy.
The physical meaning of this Hamiltonian system is at the moment
completely obscure, but it does provide us with a convenient language
for describing the transition:
The domain of the electric confinement phase lies in the asymptotic
past ($x_3\to-\infty$) where $\alpha=0$, $\beta=0$ and both the potential
and the kinetic energy vanish.
Note that $\alpha=0$ is at the maximum of the potential~\SWPotential,
so as the time $x_3$ goes on, the system slides off this `potential
hill' and both the coordinate $\alpha$ and the velocity $\beta$ begin
to grow according to the law of energy conservation
$$
K(\beta)\ +\ V(\alpha)\ =\ {\rm const}\ =\ 0.
\eqn\SWEnergyConservation
$$
Eventually, as $\alpha$ grows large, the `force' $F=-dV/d\alpha$
becomes more or less constant, $F\approx m$, and the mechanical
system ends up in free fall, $\rho\approx mx_3+\rm const$.
 
{}From the domain wall's point of view,
the free fall in the asymptotic future describes
the domain of the perturbed Coulomb phase.
Indeed, the free-fall equation $\rho\approx mx_3+\rm const$ means
$$
16\pi^2m\,x_3\ =\ {\rm const}\
+\ {\Lambda^2-U\over\Lambda^2}\,\log{32e\Lambda^2\over\Lambda^2-U}\,,
\eqn\SWeocU
$$
which agrees with the $\Lambda^2-U\ll\Lambda^2$ limit of
the Coulomb-domain formula~\SWApproxProfile.
At the same time, energy conservation~\SWEnergyConservation\ implies
$$
\alpha\ \approx\ 1+\coeff{1}{m}K(\beta)\
=\ 1\ +\ \left({\Lambda^2-U\over 4\pi\Lambda h}\right)^2
	\left(\log{32\Lambda^2\over\Lambda^2-U}\,+{1\over2}\right),
\eqn\SWeomAlpha
$$
which becomes large for $U\le\Lambda^2-O(4\pi\Lambda h)$.
Consequently,
the monopole condensate $\mono=he^{-\alpha/2}$ peters out,
exactly as it should do as one goes into the Coulomb phase domain.

The exact solution to the equations of motion~\SWEoM\ is given by the integral
$$
x_3\ = \int{d\alpha\over\beta}
\eqn\SWMotion
$$
where $\alpha$ and $\beta$ are related to each other via
eq.~\SWEnergyConservation.
Similar to the toy model, we have analytic formul\ae\ for this integral
in the asymptotic regimes of either small or large $\alpha$ but a numerical
evaluation is required for the intermediate range;
the field profiles resulting from such a numerical integration
are presented on figure~4.\figinsert{f4}
Analytically, eqs.~\SWeocU\ and \SWeomAlpha\ describe the asymptotic form
of the field profiles on the Coulomb-side tail end of the transition,
$x>-\half w+O(1/8\pi h)$ ($w\approx 0.0625 m^{-1}$ being
the domain wall's thickness in the $\Lambda\gg m$ limit);
at the confinement-phase tail end, $x<-\half w-O(1/8\pi h)$
the fields behave according to
$$
\eqalign{
U\ &\approx\ \Lambda^2\
-\ (32\Lambda^2)\, \exp\left(-\half-(6\pi h(x_0-x))^{2/3}\right) ,\cr
\mono\ &\approx\ h\
-\ (\coeff{4\sqrt{2}}{\pi}\Lambda)\, (6\pi h(x_0-x))^{1/3}\,
	\exp\left(-\half-(6\pi h(x_0-x))^{2/3}\right) ,\cr
}\eqn\SWConfiningSide
$$
for some constant $x_0\approx -\half w$.
\foot{More precisely,
    $$
    \eqalign{
    U\ &\approx\ \Lambda^2\ -\ (32\Lambda^2)\, \exp\left(\half-t^2\right)\,
	\left(1+O(e^{-t^2})\right),\cr
    \mono\ &\approx\ h\ -\ (\coeff{4\sqrt{2}}{\pi}\Lambda)\,
	t\,\exp\left(\half-t^2\right)\,\left(1+O(e^{-t^2})\right),\cr
    x\ &\approx\ -{w\over2}\ + {1\over 6\pi h}\left(
	    -(t^3-\coeff32 t) + (t_0^3-\coeff32 t_0)
	    + C_1 +O(e^{-t^2})\right),\cr
    }\eqno\SWConfiningSide'
    $$
    where $t$ is an auxiliary parameter, $t_0$ is the larger of the
    two solutions of the transcendental equation
    $$
    t_0e^{-t_0^2}=C_2{h\over\Lambda}
    $$
%    and $C_1\approx0.3103$ and $C_2\approx0.11534$
    and $C_1\approx0.31$ and $C_2\approx0.115$
    are numerical constants.
    }
%

We conclude this section with an overview of the entire Seiberg--Witten
domain wall put together.
Figure~5\figinsert{f5}
shows the profiles of the $U$, $\mono$ and $\dyon$ fields for $m=\Lambda/2000$.
Notice that the transition regions are unexpectedly thick
for such a small $m/\Lambda$ ratio.
For smaller masses, the transition regions become thicker in absolute terms
--- their thickness is $O(1/h)$ and thus increases as $1/\sqrt{m}$ ---
but the Coulomb phase domain becomes thicker at the faster rate $w\propto1/m$,
so in relative terms, the transition regions become thinner.
For example, for $m=\Lambda/2,000,000$, 96\% of the total wall's thickness
is taken by the Coulomb-phase domain while each transition region takes
only 2\%.\foot{%
    For the purpose of this comparison, we define the transition regions
    as regions in which the monopole or dyon fields change from $0.99\,h$
    on the confinement-phase side to $0.01\,h$ on the Coulomb-phase side.}
%
On the other hand, for larger $m/\Lambda$ ratios, the transitional regions
encroach even more on the Coulomb phase domain until they take over the whole
domain wall for $m\sim\Lambda/400$.
Indeed, in order to have $\alpha\gsim9$ (\ie, $\mono\lsim h/100$)
while at the same time $\Lambda^2-U\lsim\Lambda^2$, eq.~\SWeomAlpha
\foot{%
    Strictly speaking, eq.~\SWeomAlpha\ is only accurate for
    $\Lambda^2-U\ll\Lambda^2$, but we estimate the error in extrapolating
    this formula to $U\sim0$ as being no worse than about 20\%.}
requires $\Lambda\gsim 17h$ \ie,
$$
{\bf small}\ m\ {\bf means}\quad
{m\over\Lambda}\ \lsim\ {1\over 400}\,.
\eqn\SWRatioLimit
$$
As of this writing, this surprisingly stringent requirement for
the validity of the $m\to0$ picture of the SW domain wall
remains a puzzle.\foot{%
    One reason for the smallness of this limitation is the unphysical
    normalization of the holomorphic mass parameter $m$.
    In QCD-like terms, the $\Phi$ superfield describes an $SU(2)$ triplet
    of fermions and scalars whose canonically normalized running current mass is
    $$
    M_c(p^2)\ =\ {m\over g_{\Phi\overline\Phi}(p^2)}\
    =\ mg^2_{SU(2)}(p^2)\ =\ {4\pi^2 m\over\log(p^2/\Lambda^2)}\,.
    $$
    In QCD, the running stops at $p^2\sim(2\pi\Lambda)^2$;
    assuming similar pattern in the Seiberg--Witten theory, we have
    $M_c\sim 10m$.
    \subpar
    Naively, this normalization issue suggest the onset of the small-$m$
    regime of the SW theory for $m\lsim\Lambda/10$.
    Instead, the small-$m$ picture of the SW domain wall does not emerge
    until the mass $m$ becomes 40 times smaller than that;
    we do not know why.}

\endinput


==> Summary.tex <==
%auto-ignore
%
% Summary of the DomainWall paper.
%

\chapter{Summary}

Let us now summarize our discussion of the BPS-saturated domain wall
configurations.
Although their tension can be calculated exactly even in a strongly
interacting theory such as a confining $\NS=1$ SSYM, their structure
and even their very existence depend on the theory's details;
indeed, there is no rigorous proof that the domain walls of the
$\NS=1$ SSYM are BPS saturated.
Nevertheless, our investigation provides good evidence that they are
BPS and sheds much new light on their structure.
It also reveals some unexpected intricacies associated with domain walls;
hopefully, our results and observations will provide
a starting point for further study.

Rather than aiming directly at the domain walls of the $\NS=1$ SSYM,
our study was focused on two related theories, namely Seiberg--Witten
and MQCD.
Most of our work was done in the framework of the $\NS=2$ $SU(2)$
Seiberg--Witten theory perturbed by the second-SUSY-breaking
mass of the adjoint chiral superfield.
The vacuum structure of this theory follows from the effective
superpotential~\val\VYTSU\ for the gaugino and scalar condensates;
there are precisely two degenerate vacua which smoothly connect
in the low-mass limit to the two singularities of the Seiberg--Witten
moduli space where the magnetic monopoles or dyons become massless
and condense.
Likewise, in the large-scalar-mass limit, we have an effective $\NS=1$
SSYM theory with $\N=2$ degenerate vacua, and these are precisely the
vacua we get.
Nowhere in our analysis we find any sign of existence of additional,
non-chiral vacua advocated in earlier work\refmark{\KovShi}
or any kind of a phase transition;
instead, we find the same two degenerate vacua for all $m\neq0$.

For small $m\ll\Lambda$, we have not only established the existence
of a BPS saturated domain wall solution but actually calculated its
field profiles $U(x_3)$, $\mono(x_3)$ and $\dyon(x_3)$.
The profiles --- depicted on figure~5 --- show a five-layer
structure of the wall,
with two confining-phase domains at the two ends, a perturbed
Coulomb phase domain in the middle and two transition regions
between these domains.
Based upon continuity of the vacuum structure of the theory,
we argued that the BPS domain wall solution exists for all $m\neq0$
and even in the $m\to\infty$ limit of the $\NS=1$ SSYM.
The five-layer structure, however, survives only for very small
$m\lsim\Lambda/400$:
For larger masses, the two transition regions take over the whole
domain wall and soon enough we have both the magnetic monopole
condensate and the dyon condensate in the same region of space
in the middle of the wall.
Clearly this situation cannot be described in terms of an effective
local field theory such as Seiberg--Witten;
furthermore, the wall becomes so narrow that the higher-derivative
terms in the BPS equations become important.
Consequently, we could not calculate the wall's field profiles 
for larger masses; this remains an open problem for future work.

Our analysis has revealed several interesting properties of the
gaugino condensates in theories with adjoint scalars.
In vacuum states with four unbroken supercharges, the neutral photinos
do not condense and the gaugino condensate is solely due the
electrically charged winos.
However, there is a non-trivial photino condensate in the middle of a
BPS domain wall which breaks two more supercharges and leaves only two
supercharges unbroken.
Furthermore, for small $m$, the charged winos condense outside the wall
and near its ends, but deep inside the wall the charged
 winos do not even exist.
For larger $m$, both the photino and the wino condensates exist
throughout the domain wall but follow qualitatively different profiles.
(Except in the effectively scalar-less $\NS=1$ SSYM theory
for very large $m$ where the very distinction between the winos
and the photinos becomes unphysical.)

In the course of our investigation into the Seiberg--Witten domain walls,
we encountered several surprises.
Among the surprising features which we do not fully understand and
which deserve future attention are:
the amazing accuracy of the approximation~\val\SWApproxMetric,
the stringency of the limit~\val\SWRatioLimit\ for the validity
of the low-mass approximation and
the Hamiltonian form of the BPS equations~\val\SWEoM\
for the transitional regions;
indeed, the physical meaning of the Hamiltonian
$\rm \SWKinetic+\SWPotential$ remains completely obscure.
In addition, there is plenty of open questions pertaining to
the $SU(\N>2)$ theories we have not explored in this article,
for example, the issue of the superpotential cusps\refmark{\KovShiSmi}
for $\N>2$.
However, following the work of Douglas and Shenker,\refmark{\val\DS}
we expect significant simplification of the problem in the large
$\N$ limit.
We are currently investigating such large-$\N$ domain walls and have
some preliminary results for the extremely low mass, almost $\NS=2$
Seiberg--Witten regime of the $SU(\N)$ theory.
In particular, we find the same five-layer structure of the BPS
domain walls as in the $SU(2)$ case and even the Hamiltonian form
of the BPS equations in the transition regions.
Furthermore, we confirm Witten's result\refmark{\WittenQCD} that
the wall's tension is proportional to $\N$
(rather than $\N^2$ one naively expects from a solitonic solution).

We have also tried --- with limited success --- to investigate
the BPS domain walls in MQCD.
We have translated Witten's geometrical picture\refmark{\WittenMQCD}
of such walls into an explicit set of partial
differential equations.
We also managed to greatly simplify these equations for some special cases.
In particular, for the MQCD analogue of the $\NS=1$ $SU(2)$ SSYM theory,
we ended up with a single fourth-order Monge--Ampere equation for one
real function.
Unfortunately, we could not solve this equation for the domain-wall
boundary conditions;
also the known mathematical theorem assuring that some Monge--Ampere
equations always have a solution does not apply to the specific
equation and boundary conditions at hand.
Nevertheless, by analogy with the Seiberg--Witten theory, the MQCD
most likely does have a BPS domain wall solution we simply have not
found yet.
Thus, our results make a good starting point for future work;
when the solution will be eventually found, it is likely to
teach us much about the domain walls in both quantum field theory
and string/M theory.


\par\smallskip
\noindent \undertext{Acknowledgements:}\quad
The authors wish to thank A.~Brandhuber, N.~Itzhaki and S.~Theisen
for many fruitful discussions of domain walls in MQCD.
%Much of the present work was accomplished while 
%V.~K.\ was visiting Tel-Aviv University and J.~S. the university of
%Texas, Austin. We thank  US-Israeli Binotional Science Foundation for
%funding those visits. 
An important part of the work  was accomplished while
V.~K.\ was visiting
the ITP at Santa Barbara; many thanks for the hospitality.

\endinput


==> Titlepage.tex <==
%auto-ignore
%% Title page of the DomainWall paper

\Pubnum={UTTG--16--98\crcr TAUP--2532--98}
%\draft
\date{November 22, 1998}
\titlepage
\title{Domain Walls in Supersymmetric Yang--Mills Theories
\foot{Research supported in part by
	the US--Israeli Binational Science Foundation,
	the US National Science Foundation (V.~K., grant \#PHY--95--11632),
	the Robert A.~Welsh Foundation (V.~K.).}%
    }
\author{Vadim S.\ Kaplunovsky,\attach*\break
	Jacob Sonnenschein\attach\dagger and Shimon Yankielowicz\attach\dagger}
\smallskip
\leftline{\tenit\quad$*$ Theory Group, Physics Dept.,
	University of Texas, Austin, TX 78712, USA}
\leftline{\tenit\quad$\dagger$ School of Physics and Astronomy,
	Tel Aviv University, Ramat Aviv, Tel Aviv 69978, Israel}
\vfil

\abstract
We study BPS saturated domain walls in the supersymmetric $SU(2)$ gauge theory.
For a theory with a very light adjoint scalar (mass $m\lsim\Lambda/400$)
we use the perturbed $\NS=2$ Seiberg--Witten theory to calculate the
actual field configuration of the domain wall.
The wall has a sandwich-like five-layer structure of three distinct phases
--- electric confinement, Coulomb and oblique confinement ---
separated by two separate transition regions.
%
For larger scalar masses, the three-phase structure disappears and the
Seiberg--Witten theory becomes inadequate because of two major problems:
First, the higher-derivative interactions between the light fields become
relevant and second,
both the magnetic monopole condensate and the dyon condensate show up
in the same region of space, a phenomenon indescribable in terms of a local
field theory.
Nevertheless, we argue that the BPS saturated domain wall continues to
exist in this regime and give a qualitative description of the scalar
and gaugino condensates.
%
Finally, we discuss the domain walls in MQCD and translate the BPS conditions
into coupled non-linear differential equations.

\endpage
\endinput



==> ToyModel.tex <==
%auto-ignore
%
% Section 3 of the DomainWall paper
%
\chapter{A Toy Model}
%
In order to see how the small $m$ and the large $m$ regimes of the
BPS domain wall differ from each other,
let us now consider a simplified toy model of the Seiberg--Witten
theory in which both regimes are governed by an easy to understand
local $\NS=1$ supersymmetric effective field theory.
Specifically, let us replace
the electric and the magnetic charges of the SW theory with
two different kinds of electric charges.
That is, our model has a $U(1)\times U(1)$ gauge symmetry
and the analogues of the monopole, the anti-monopole, the dyon
and the anti-dyon have the following purely electric charges:
$\mod^{(0,0)}$, $\mono^{(+1,0)}$, $\amono^{(-1,0)}$, $\dyon^{(+1,+1)}$
and $\adyon^{(-1,-1)}$;
there are no magnetic charges in this model.
For simplicity, we set the Fayet-Iliopoulos D-terms for the two $U(1)$
factors to zero while the superpotential is a simplified version of
\SWMagneticW\ combined with \SWDyonicW, namely
$$
W = (\mod-\Lambda)\mono\amono\ +\ (\mod+\Lambda)\dyon\adyon\ - h^2\mod\,.
\eqn\ToyW
$$
where $\mod$ is a linearized analogue of the SW modulus $U$
and $h^2\sim m\Lambda$.

The phase structure of our model is analogous to that of the SW
theory, except for the extra massless photon.
For $h=0$ (but $\Lambda\neq0$), the model is similar to the SW
theory with the unbroken $\NS=2$ SUSY:
There is a continuous family of
degenerate vacua parametrized by the expectation value of the $\mod$ field.
For generic values of $\vev\mod$, the only massless particles are the two
photons and the $\mod$ field (and their superpartners), but
for $\vev\mod=\pm\Lambda$, there are additional massless charged particles,
namely $\mono$ and $\amono$ or $\dyon$ and $\adyon$.
On the other hand, for $h\neq0$, the model behaves like the SW theory with
supersymmetry broken down to $\NS=1$:
There are two discrete but degenerate vacua,
$$
\eqalign{
(1)\quad &
\mod=+\Lambda,\quad\mono=\amono=h,\quad\dyon=\adyon=0\cr
{\rm and\ }(2)\quad &
\mod=-\Lambda,\quad\dyon=\adyon=h,\quad\mono=\amono=0.\cr
}\eqn\TwoVacua
$$
Furthermore, while each vacuum leads to one massless and one massive
photon, these two vacua lead to Higgsing of  different linear combinations
of the two $U(1)$ gauge fields;
this is analogous to the two vacua of the SW theory leading respectively
to {\sl electric confinement \it v.\ \sl oblique confinement}.

Notice that the superpotential~\ToyW\ is single-valued
and our toy model gives rise to the two vacua~\TwoVacua\
without any help from some `hidden' heavy degrees of freedom;
consequently, the domain-wall solution interpolating between the
two vacua can be analyzed in terms of straightforward
field equations of motion.
For a BPS-saturated domain wall, these equations follow from
the requirement of preserving two out of four global supercharges
of the $\NS=1$ theory, namely
$$
\left(Q_\alpha -ie^{i\varphi} \sigma^3_{\alpha\dot\alpha}
	{\overline Q}\vphantom{Q}^{\dot\alpha}\right)
\ket{\rm wall}\ =\ 0
\eqn\PreservedQ
$$
where the $x_3$ coordinate axis is normal to the wall
(\ie, the wall lies in the $(x_1,x_2)$ plane)
and $\varphi=\arg(\Delta W$ between the two vacua).
%
In terms of the bosonic fields of an effective field theory
and their auxiliary superpartners
(generically denoted $A^i$, $V^a_\mu$ and $F^i$, $D^a$,
respectively),
eqs.~\PreservedQ\ imply
$$
\displaylines{
V^a_\mu(x_3)\ \equiv\ 0,\qquad D^a(x_3)\ \equiv\ 0,\qquad\cr
{}\hfill{}{dA^i\over dx_3}\
=\ e^{i\varphi} F^i\
\equiv\ e^{i\varphi} g^{i\bar\jmath}\,
	\partder{W^*}{\overline{A}\vphantom{A}^{\bar\jmath}}
\hfill\eqname\BPSWall\cr
}$$
(in the axial gauge $V^a_3\equiv0$),
$g^{i\bar\jmath}$ being the inverse of the
quantum-corrected K\"ahler metric $g_{j\bar\imath}(A,A^*)$
of the scalar-field space.

For simplicity, let us take the K\"ahler metric of our toy model to be flat,
$g_{j\bar\imath}\equiv\delta_{j\bar\imath}$
(in spite of any quantum corrections).
Consequently, eqs.~\BPSWall\ for our model become
$$
\eqalign{
\omit\span\mono\ \equiv\ \amono,\qquad \dyon\ \equiv\ \adyon,\cr
{d\mono\over dx_3}\ &
=\ e^{i\varphi}\,\amono^*(\mod-\Lambda)^*,\cr
{d\dyon\over dx_3}\ &
=\ e^{i\varphi}\,\adyon^*(\mod+\Lambda)^*,\cr
{d\mod\over dx_3}\ &
=\ e^{i\varphi}\left(\mono\amono+\dyon\adyon-h^2\right)^*,\cr
}\eqn\BPSToy
$$
where $\varphi=\arg(\Delta W=2\Lambda h^2)$, assuming
the domain wall solution asymptotes to the first vacuum of \TwoVacua\
for $x\to-\infty$ and to the second vacuum for $x\to+\infty$.

Eqs.~\BPSToy\ and \TwoVacua\ are invariant under global phase changes
$$
\displaylines{
\mono\ \to\ e^{i\beta}\mono,\quad
\amono\ \to\ e^{i\beta}\amono,\quad
\dyon\ \to\ e^{i\beta}\dyon,\quad
\adyon\ \to\ e^{i\beta}\adyon,\quad
h\ \to e^{i\beta}h,\cr
\mod\ \to\ e^{i\gamma}\mod,\quad
\Lambda\ \to\ e^{i\gamma}\Lambda,\cr
}$$
so without loss of generality we take the parameters $h$ and $\Lambda$
to be real and positive.
Another important symmetry is the charge conjugation, which
(for real $h$ and $\Lambda$) acts on all the scalar fields of the theory
by complex conjugation.
Since a BPS-saturated domain wall
between two given vacua should be unique (if it exists at all),
%\Vnote{I {\sl think} this is true, but I am not totally sure.
%	We need a reference or a a good argument for this statement.}
%
we should look for a solution in which all fields are {\sl real}
functions of the $x_3$ coordinate.

Solving eqs.~\BPSToy\ for the real fields is a fairly straightforward procedure.
First, the equations for the $\mono$ and $\dyon$ fields imply
$$
{d\over dx_3}\,\log(\mono\dyon)\ =\ 2\mod,\qquad
{d\over dx_3}\,\log{\dyon\over\mono}\ =\ 2\Lambda,
\eqn\TwoEqs
$$
which allows us to express the entire field configuration in terms of
just one real function $\xi(x_3)$ according to
$$
\eqalign{
\mono(x_3)\ =\ \amono(x_3)\ &
=\ h\exp\left( -\half\xi(x_3)\,-\,\Lambda x_3 \right),\cr
\dyon(x_3)\ =\ \adyon(x_3)\ &
=\ h\exp\left( -\half\xi(x_3)\,+\,\Lambda x_3 \right),\cr
\mod(x_3)\ &
=\ -{1\over2}\,{d\xi\over dx_3}\,.\cr
}\eqn\xiAnsatze
$$
(Without loss of generality, we have placed the origin of the $x_3$
coordinate in the middle of the wall.)
In terms of the $\xi(x_3)$, eq.~\BPSToy\ for the $\mod$ field becomes
$$
\eqalign{
{d^2\xi\over dx_3^2}\ &
=\ -2\,{d\mod\over dx_3}\
	=\ 2\left(h^2-\mono^2-\dyon^2\right)\cr
&=\ 2h^2\left( 1\,-\,2\cosh(2\Lambda x_3)\exp(-\xi)\right) ,
}\eqn\xiEq
$$
while the boundary conditions
$$
\xi(x_3\to\pm\infty)\ =\ 2\Lambda|x_3|
\eqn\xiBC
$$
assure the field configuration asymptotically approaches the
vacua \TwoVacua\ as one goes away from the domain wall.

{}From the general form of eq.~\xiEq, it is clear that there is a
unique solution $\xi(x_3)$ for any $h,\Lambda>0$, although for
generic values of $h$ and $\Lambda$, the solution
is not expressible in closed form in terms of familiar functions.
However, for the special case of $h^2=2\Lambda^2$,
the solution simplifies to
$$
\xi(x_3)\ =\ 2\log\left(2\cosh\Lambda x_3\right)
\eqno\eq
$$
and hence
$$
\eqalign{
\mono\ =\ \amono\ &
=\ {h\over1+e^{2\Lambda x_3}}\,,\cr
\dyon\ =\ \adyon\ &
=\ {h\over1+e^{-2\Lambda x_3}}\,,\cr
\mod\ &
=\ -\Lambda\tanh\Lambda x_3\,.\cr
}\eqn\MidddleSolution
$$
Similarly, in the limit $h\gg\Lambda$, the solution becomes
$$
\xi(x_3)\ \approx\ \log\left(2\cosh2\Lambda x_3\right)
\eqno\eq
$$
and hence
$$
\eqalign{
\mono\ =\ \amono\ &
\approx\ {h\over\sqrt{1+e^{4\Lambda x_3}}}\,,\cr
\dyon\ =\ \adyon\ &
\approx\ {h\over\sqrt{1+e^{-4\Lambda x_3}}}\,,\cr
\mod\ &
\approx\ -\Lambda\tanh2\Lambda x_3\,.\cr
}\eqn\HeavySolution
$$
The two solutions are plotted in Figure~1,
\figinsert{f1}
which shows their qualitative similarity to each other;
both walls have similar distance scales $O(1/\Lambda)$ that
govern the $x_3$ dependence of all the fields and there
are no interesting features at either longer or shorter distances.
Naturally, we expect the same behavior from the domain wall
for any $h\gsim O(\Lambda)$.

On the other hand,
the $h\ll\Lambda$ regime of the domain wall solution is very different.
Indeed, assuming a rather mild inequality
$$
\exp\left( {\Lambda^2\over h^2}\right)\ \gg\ 1,
\eqn\LightAssumption
$$
we approximate eq.~\xiEq\ as
\foot{%
    This approximation is based upon the lower bound
    $\xi>(\Lambda/h)^2$ (which follows from
    ${d^2\xi\over dx_3^2}<2h^2$ while $\xi\ge2\Lambda|x_3|$).
    Consequently, the assumption~\LightAssumption\ implies
    $e^{\xi}\gg1$ and hence $1-2\cosh(2\Lambda x_3)\exp(-\xi)=
    1-\exp(2\Lambda|x_3|-\xi)-\exp(-2\Lambda|x_3|-\xi)\approx
    1-\exp(2\Lambda|x_3|-\xi)$.
    }
$$
{d^2\xi\over dx_3^2}\
\approx\ 2h^2\left( 1-\exp(2\Lambda|x_3|-\xi)\right) ,
\eqn\xiApproxEq
$$
which can be solved in terms of the integral equation
$$
2h|x_3|\ =\ \int_{\xi(x_3)-2\Lambda|x_3|}^{\sigma_0}\,
{d\sigma\over\sqrt{\sigma+e^{-\sigma}-1}}\,,
\eqn\IntEq
$$
where $\sigma_0+e^{-\sigma_0}-1=(\Lambda/h)^2$;
in light of the assumption~\LightAssumption,
$\sigma_0\approx(\Lambda/h)^2+1$.
The integral in eq.~\IntEq\ can be evaluated explicitly
whenever its lower limit $\xi(x_3)-2\Lambda|x_3|$ is either
large or small, which leads to
$$
\xi(x_3)\ =\ {\Lambda^2\over h^2}\ +\ h^2x_3^2\ +\ 1\
+\ O\left(\exp\left[-\left(\coeff{\Lambda}{h}-h|x_3|\right)^2\right]\right)
\eqn\InnerRegion
$$
for $|x_3|< \Lambda h^{-2} - O(h^{-1})$ and
$$
\eqalignno{
\xi(x_3)\ =\ 2\Lambda|x_3|\ &
+\ 2C\exp\left[-\sqrt{2}h\left(|x_3|-\Lambda h^{-2}\right)\right]\cr
&+\ O\left(\exp\left[-2\sqrt{2}h\left(|x_3|-\Lambda
	h^{-2}\right)\right]\right) &
\eqname\OuterRegions\cr
}$$
($C\approx0.3312$ is a numerical constant)
for $|x_3|> \Lambda h^{-2} + O(h^{-1})$.
In the intervening ranges of $x_3$ near $\pm\Lambda h^{-2}$,
$$
\xi(x_3)\ \approx\ 2\Lambda|x_3| +\ O(1)\quad
{\rm for} \left| |x_3|-\Lambda h^{-2}\right| \lsim O(h^{-1})
\eqn\MessyRegions
$$
but a numerical evaluation of the integral~\IntEq\ is required for a
more accurate answer.
Figure~2\figinsert{f2}
shows the field profiles resulting from such
a numerical integration.

Altogether, the domain wall of the model with $h\ll\Lambda$ has
a five-layer sandwich-like configuration:
\pointbegin %1
The Left Asymptotic region at $x_3<-\Lambda h^{-2}-O(h^{-1})$ where
$$
\eqalign{
\mono\ =\ \amono\ &
\approx\ h\ -\ Ch\exp\left(-\sqrt{2}h(|x_3|-\Lambda h^{-2})\right),\cr
\dyon\ =\ \adyon\ &
\approx\ h\exp\left(-2\Lambda|x_3|\right)\ \approx\ 0\cr
{\rm and}\quad \mod\ &
\approx\ \Lambda\
    -\ \sqrt{2}Ch\exp\left(-\sqrt{2}h(|x_3|-\Lambda h^{-2})\right).\cr
}\eqn\LeftTail
$$
This is the exponential tail of the domain wall into the domain
of the electric confinement phase
\foot{We name the phases of our toy model after their SW analogues.
    Likewise, we call $\mono$ the `monopole' field, $\dyon$ the `dyon',
    \etc, \etc
    }
at $x_3\to-\infty$.

\point %2
The Left Transitional region at
$-O(h^{-1})< x_3+\Lambda h^{-2}<+O(h^{-1})$
where
$$
\mod\approx\Lambda-O(h),\qquad
\dyon=\adyon=O(e^{-\Lambda^2/h^2})\approx0,\qquad
\mono=\amono=O(h)\qquad
\eqn\LeftTransition
$$
but the exact profiles of the $\mono(x_3)$ and $\Lambda-\mod(x_3)$
are rather complicated.
Qualitatively, the monopole fields $\mono$ and $\amono$ `switch off'
\ie, decrease from $h$ to almost zero while the $\mod$ field does not
deviate far from its vacuum value $+\Lambda$ (note $\Lambda\gg h$);
the dyon fields $\dyon$ and $\adyon$ remain negligible throughout
this region.

\point %3
The Middle Layer at
$-\Lambda h^{-2}+O(h^{-1})<x_3<+\Lambda h^{-2}-O(h^{-1})$ where
$$
\eqalign{
\mono\ =\ \amono\ &
\approx\ h\exp\left( -h^2\left(x_3+\Lambda h^{-2}\right)^2\right)\
	\approx\ 0,\cr
\dyon\ =\ \adyon\ &
\approx\ h\exp\left( -h^2\left(x_3-\Lambda h^{-2}\right)^2\right)\
	\approx\ 0\cr
{\rm and}\quad \mod\ &
\approx\ -h^2\,x_3\,.\cr
}\eqn\MiddleLayer
$$
In this layer, both the monopole and the dyon fields are negligible
while the modulus field $\mod$ {\sl slowly} interpolates between
its two vacuum values $+\Lambda$ and $-\Lambda$.

\point %4
The Right Transitional region at
$-O(h^{-1})< x_3-\Lambda h^{-2}<+O(h^{-1})$
where the `monopole' fields are negligible, the modulus $\mod$
is close to its expectation value $-\Lambda$ in the domain
of the oblique confinement phase
and the dyon fields $\dyon$ and $\adyon$ `switch on' \ie, increase
from almost zero to almost $h$,
$$
\mono=\amono=O(e^{-\Lambda^2/h^2})\approx0,\qquad
\mod\approx-\Lambda+O(h),\qquad
\dyon=\adyon=O(h).\qquad
\eqn\RightTransition
$$

\point %5
The Right Asymptotic region at $x_3>+\Lambda h^{-2}+O(h^{-1})$
or the exponential tail of the domain wall into the oblique confinement
domain at $x_3=+\infty$.

Notice that for $h\ll\Lambda$,
the characteristic length scale $O(1/h)$ of significant field change
in the two transition regions (2 and 4 above)
is much shorter than the thickness
$2\Lambda/h^2$ of the middle layer (3) of the domain wall.
Indeed,
in the $h\to0$ limit of the wall, the middle layer becomes so thick
that it acts almost like a separate phase of the theory, greatly
resembling the `Coulomb' phase of the $h=0$ model 
where $\vev\mono=\vev{\smash\amono\vphantom\mono}
=\vev\dyon=\vev{\smash\adyon\vphantom\dyon}=0$ while
the modulus field $\mod$ has an arbitrary vacuum expectation value.
{\sl In bulk}, this Coulomb phase becomes energetically unstable
--- as well as non-supersymmetric --- in presence of a non-zero
O'Raighfeartaigh F-term $h^2\mod$, however small,
but {\sl in a layer of a finite thickness}, a small O'Raighfeartaigh
term is just an adiabatic perturbation that
turns on a gradient $\nabla\mod=-h^2$ of the modulus field.
The perturbed Coulomb phase remains stable and invariant under
two out of four supercharges --- and clearly this is precisely
the field configuration in the middle layer \MiddleLayer\
of the $h\ll\Lambda$ domain wall.

Altogether, our field configuration is best thought of
not as two phases separated by a multi-layer domain wall
but rather as a sequence of {\it three domains of distinct phases}
separated by two transitional regions.
In SW-inspired terminology, the three phases are respectively the
electric confinement phase, the perturbed
Coulomb phase and the oblique confinement phase;
the two confining phases extend to $x_3=\mp\infty$ while
the perturbed Coulomb phase has a finite thickness $2\Lambda h^{-2}$.
The two transition regions between either confining phase and the
(perturbed) Coulomb phase are in a sense domain walls
on their own rights, well separated
from each other and from the other confining phase
and much thinner than the Coulomb phase domain between them.

Clearly, this three-phase structure of a
BPS-saturated domain wall is by no means
a peculiar feature of our toy model.
Instead, it is generic to all theories where a continuous family of
exactly degenerate vacua collapses
to several isolated vacua when one adds {\it small} F-terms $W_F$ for the
moduli fields of the theory (\eg, $W_F=h^2\mod$):
As long as such F-terms are small, the adiabatic perturbation of the
generic-moduli phase (\eg, the Coulomb phase of the SW theory or our
toy model) is stable and invariant under two supercharges in a layer
of a finite thickness in which the moduli fields have
gradients $\nabla\mod^i=
e^{i\varphi}g^{i\bar\jmath}(\partial W_F/\partial\mod^j)^*$
(\cf~eq.~\BPSWall).
Within the domain of this phase, one may ignore the fields that become
light only at some special points or subspaces of the moduli space.

In all such theories, a BPS domain wall between two bulk-stable
phases has a three-domain structure with the (perturbed) generic-moduli
phase occupying the middle domain.
The relatively thin (for small O'Raighfeartaigh terms)
transition regions between this domain and the bulk-stable phases
on either side of the domain wall
are characterized by moduli fields having
values within $O(h)$ of the appropriate bulk-stable phase's VEVs
and also by non-trivial values of the light fields and
condensates present in that particular phase
(\eg, {\sl either} $\mono$ and $\amono$ {\sl or} $\dyon$ and $\adyon$).
However, one may safely ignore the fields that become light in any
other phase of the theory;
for example, in the toy model, the $\dyon$ and $\adyon$ fields play no role
in the transition between the Coulomb and the electric-confinement phases
while the $\mono$ and $\amono$ fields are as good as absent from
the Coulomb-to-the-oblique-confinement transition region.

The above picture describes the $h\ll\Lambda$ regime of {\sl small}
O'Raighfeartaigh terms, but increasing $h$ gives rise to two major
complications:
First, perturbing the generic-moduli phase too strongly may change its
nature;
indeed, the $O(h^2)$ gradients of the moduli amount to a momentum, so
all particles with masses up to $O(h^2/\Lambda)$ should be included
in the effective theory.
Second, the $O(\Lambda/h^2)$ thickness of the middle domain shrinks with $h$
at a faster rate 
than the $O(1/h)$ characteristic length scale of the transition regions.
Eventually, for $h=O(\Lambda)$, the middle domain disappears under the
(inner) tail ends of the two transition regions and the latter merge
into a single featureless wall where all fields are present more or less
throughout the wall's thickness.
For example, in our toy model, both `monopole' and `dyon' fields have
$O(h)$ values in the middle of the domain wall, \cf~figure~1.
Generically, in a more complicated theory with a similar three-domain
structure of a BPS domain wall in the $h\ll\Lambda$ regime,
we expect the $h\ge O(\Lambda)$ regime of the wall to be quite different.

\endinput


==> f1.tex <==
%auto-ignore

% Figure 1 for the DomainWall paper
$$
\dimen0=\displaywidth
\divide\dimen0 by 16
\vbox{
    \hsize=14\dimen0
    \line{%
	\beginpicture
	    \setcoordinatesystem units <\dimen0,3cm>
	    \setplotarea x from -3.05 to 3.6 , y from -0.75 to 1.1
	    \arrow <10pt> [0.1,0.3] from -3.05 0 to +3.2 0
	    \put {$x_3$} [lB] <2pt,2pt> at 3.2 0
	    \putrule from 0 -0.75 to 0 +1.1
	    \setquadratic
	    \PLOT "f1a-M"
	    \put {$\mono$} [lt] <2pt,-2pt> at -3 1
	    \setcoordinatesystem point at 0 0
	    \PLOT "f1a-D"
	    \put {$\dyon$} [rt] <-3pt,-2pt> at 3 1
	    \setcoordinatesystem units <\dimen0,2.12cm> point at 0 0
	    \PLOT "f1a-T"
	    \put {$\mod$} [rb] <-3pt,2pt> at 3 -1
	    \endpicture
	\hskip 2em plus 2fil minus 0.5em
	\beginpicture
	    \setcoordinatesystem units <\dimen0,3cm>
	    \setplotarea x from -2.55 to 3.1 , y from -0.75 to 1.1
	    \arrow <10pt> [0.1,0.3] from -2.55 0 to +2.7 0
	    \put {$x_3$} [lB] <2pt,2pt> at 2.7 0
	    \putrule from 0 -0.75 to 0 +1.1
	    \setquadratic
	    \PLOT "f1b-M"
	    \put {$\mono$} [lt] <2pt,-2pt> at -2.5 1
	    \setcoordinatesystem point at 0 0
	    \PLOT "f1b-D"
	    \put {$\dyon$} [rt] <-3pt,-2pt> at 2.5 1
	    \setcoordinatesystem units <\dimen0,1.2cm> point at 0 0
	    \PLOT "f1b-T"
	    \put {$\mod$} [rb] <-3pt,2pt> at 2.5 -1
	    \endpicture
    }
    \hrule height 0pt
    \Tenpoint
    \bigskip\noindent
    Figure~1:
    \sl Field profiles for the domain wall solution of the toy model.
    The profiles on the left picture correspond to $h^2=2\Lambda^2$;
    on the right picture, $h\gg\Lambda$.
    Note the similarity of the two pictures.
    \par
    }
$$
\endinput


==> f2.tex <==
%auto-ignore

% Figure 2 for the DomainWall paper
$$
\dimen0=0.25\displaywidth
\dimen1=3cm
\def\xrange{1.6}
\vbox{
    \hsize=0.8\displaywidth
    \beginpicture
	\setcoordinatesystem units <\dimen0,\dimen1>
%	\setplotarea x from {-\xrange} to {+\xrange}, y from -1.4 to 1.05
	\arrow <10pt> [0.1,0.3] from {-\xrange} 0 to {+\xrange} 0
	\putrule from -1 0 to -1 -0.05
	\putrule from +1 0 to +1 -0.05
	\put {$x_3$} [Bl] <0.25em,2pt> at {+\xrange} 0
	\put {\hbox to 0pt{\hss\tenpoint$-\Lambda/h^2$\hss}}
		<3pt,-3pt> [tl] at -1 -0.05
	\put {\hbox to 0pt{\hss\tenpoint$+\Lambda/h^2$\hss}}
		<3pt,-3pt> [tl] at +1 -0.05
	\put 0 <3pt,-3pt> [tl] at 0 -0.03
	\putrule from 0 -0.21 to 0 1.05
	\put {\hbox to 0pt{\hss\tenpoint$\approx$\hss}} [bl] at 0 -0.25
	\putrule from 0 -1.4 to 0 -0.25
	\setdots
	\setlinear
	\plot {-\xrange} 1 {+\xrange}  1 /
	\setsolid
	\putrule from -0.04 1 to +0.04 1
	\put {$h$} [Bl] <3pt,-3pt> at 0.05 1
	\setquadratic
	\PLOT "f2-D"
	\put {$\dyon$} [tr] <-15pt,-5pt> at {+\xrange}  1
	\PLOT "f2-M"
	\put {$\mono$} [tl] <15pt,-5pt> at {-\xrange} 1
	\setdots
	\setlinear
	\plot {-\xrange} -0.35 {+\xrange}  -0.35 /
	\plot {-\xrange} -1.35 {+\xrange}  -1.35 /
	\setsolid
	\putrule from -0.04 -0.35 to +0.04 -0.35
	\put {$+\Lambda$} [Bl] <0pt,-3pt> at 0.05 -0.35
	\putrule from -0.04 -1.35 to +0.04 -1.35
	\put {$-\Lambda$} [Bl] <0pt,-3pt> at 0.05 -1.35
	\putrule from -0.04 -0.85 to +0.05 -0.85
	\put 0 [Bl] <9pt,-3pt> at 0.05 -0.85
	\put {$\mod$} [tr] <15pt,-5pt> at {-\xrange} -0.35
	\setcoordinatesystem units <\dimen0,0.5\dimen1> point at 0 1.7
	\setquadratic
	\PLOT "f2-T"
    \endpicture
    \par \bigskip \noindent
    Figure 2:
    \sl The domain wall profile for the toy model with $\Lambda=5h$ shows
    the five-layer structure of the $\Lambda\gg h$ limit.
    \par
}
$$
\endinput


==> f3.tex <==
%auto-ignore

% Figure 3 for the DomainWall paper.
$$
\dimen0=0.45\displaywidth
\dimen1=4cm
\hbox{\Tenpoint
    \valign{%
	\vfil#\vfil\bigskip &\hrule height 0pt #\vfil\cr
	\beginpicture
	    \setcoordinatesystem units <0.4\dimen0,12.5\dimen1>
	    \setplotarea x from -1 to +1 , y from 0 to 0.08
	    \setdots \grid {10} {8} \setsolid
	    \arrow <10pt> [0.1,0.3] from -1.1 0 to 1.25 0
	    \arrow <10pt> [0.1,0.3] from 0 0 to 0 0.09
	    \putrule from -1 0 to -1 -0.004
	    \putrule from +1 0 to +1 -0.004
	    \put {\hbox to 0pt{\hss$-\Lambda^2$\hss}}
		 [tl] <2pt,-2pt> at -1 -0.004
	    \put {\hbox to 0pt{\hss$+\Lambda^2$\hss}}
		 [tl] <2pt,-2pt> at +1 -0.004
	    \put 0 [tl] <-2pt,-3pt> at 0 -0.004
	    \put {$U$} [Bl] <3pt,0pt> at 1.25 0
	    \put {$g_{U\overline{U}}$} [Bl] <3pt,0pt> at 0 0.09
	    \setquadratic
	    \PLOT "f3a-g"
	    \setdashes
	    \PLOT "f3a-gth"
	    \endpicture
	&
	\par\hsize=\dimen0
	\leftskip=-0.02\dimen0
	\rightskip=0pt plus 0.2em
	\noindent Figure 3a:
	{\sl Metric for the Seiberg--Witten modulus $U$.\/}
	The solid line plots the actual metric~\val\SWMetric,
	the dashed line --- the approximate metric~\val\SWApproxMetric;
	the metric
	$g_{U\overline U}$ is in units of $0.01\Lambda^{-2}$ per grid line.
	\par
	\cr
	\noalign{\hskip 0.2\dimen0}
	\beginpicture
	    \setcoordinatesystem units <0.135\dimen0,0.5\dimen1>
	    \setplotarea x from -3 to 3, y from -1 to 1
	    \setdots
	    \axis bottom invisible
		ticks length <0pt> andacross numbered from -3 to +3 by 1 /
	    \axis left invisible
		ticks length <0pt> andacross quantity 9 /
	    \setsolid
	    \arrow <10pt> [0.1,0.3] from -3 0 to 3.6 0
	    \put {\twelvepoint$x_3$} [Bl] <3pt,0pt> at 3.6 0
	    \arrow <10pt> [0.1,0.3] from 0 -1.05 to 0 1.3
	    \put {$U$} [Bl] <3pt,-3pt> at 0 1.3
	    \put {$+\Lambda^2$} [Bl] <3pt,-2.5pt> at +3 +1
	    \put {$-\Lambda^2$} [Bl] <3pt,-2.5pt> at +3 -1
	    \setquadratic
	    \PLOT "f3b-U"
	    \endpicture
	&
	\par\hsize=\dimen0
	\rightskip=0pt plus 0pt minus 5pt
	\noindent Figure 3b:
	{\sl Field profile $U(x_3)$ for the perturbed Coulomb domain
	inside the Seiberg--Witten domain wall (for $m\ll\Lambda$);\/}
	the $x_3$ is in units of $1/8\pi^2m$.
	\par
	\cr
	}%
    }
$$
\endinput


==> f4.tex <==
%auto-ignore

% Figure 4 for the DomainWall paper
$$
\dimen0=0.8\displaywidth
\vbox{
    \hsize=\dimen0
    \beginpicture
	\setcoordinatesystem units <0.35\dimen0,3cm>
	\arrow <10pt> [0.1,0.3] from 0 0 to 2.7 0
	\put {$x_3$} [lB] <2pt,2pt> at 2.7 0
	\setlinear\setdots
	\putrule from 0 1 to 1.8 1
	\put {$h$} [lB] <2pt,-3pt> at 1.8 1
	\setquadratic\setsolid
	\PLOT "f4-M"
	\put {$\mono$} [lt] <3pt,-3pt> at 0 1
	\setcoordinatesystem units <0.35\dimen0,5cm>
	\setlinear\setdots
	\putrule from 0 1 to 2.5 1
	\put {$\Lambda$} [lB] <2pt,-3pt> at 2.5 1
	\setquadratic\setsolid
	\PLOT "f4-U"
	\put {$U$} [lt] <3pt,-3pt> at 0 1
	\endpicture
    \hrule height 0pt
    \Tenpoint \bigskip\noindent
    Fugure~4:
    \sl Field profiles for the transitional region of the Seiberg--Witten
    domain wall ($m=\Lambda/2000$).
    The electric-confinement domain is to the left of the plot, the Coulomb
    domain is to the right.
    \par
    }
$$
\endinput



==> f5.tex <==
%auto-ignore

% Figure 2 for the DomainWall paper
$$
\dimen0=0.1\displaywidth
\dimen1=3cm
\def\xrange{4}
\def\wid{2.46}
\vbox{
    \hsize=0.8\displaywidth
    \beginpicture
	\setcoordinatesystem units <\dimen0,\dimen1>
	\arrow <10pt> [0.1,0.3] from {-\xrange} 0 to {+\xrange} 0
	\putrule from {-\wid} 0 to {-\wid} -0.05
	\putrule from {+\wid} 0 to {+\wid} -0.05
	\put {$x_3$} [Bl] <0.25em,2pt> at {+\xrange} 0
	\put {\hbox to 0pt{\hss\tenpoint$-w/2$\hss}}
		<3pt,-3pt> [tl] at {-\wid} -0.05
	\put {\hbox to 0pt{\hss\tenpoint$+w/2$\hss}}
		<3pt,-3pt> [tl] at {+\wid} -0.05
	\put 0 <3pt,-3pt> [tl] at 0 -0.03
	\putrule from 0 -0.21 to 0 1.05
	\put {\hbox to 0pt{\hss\tenpoint$\approx$\hss}} [bl] at 0 -0.25
	\putrule from 0 -1.4 to 0 -0.25
	\setdots
	\setlinear
	\plot {-\xrange} 1 {+\xrange}  1 /
	\setsolid
	\putrule from -0.04 1 to +0.04 1
	\put {$h$} [Bl] <3pt,-3pt> at 0.05 1
	\setquadratic
	\PLOT "f5-D"
	\put {$\dyon$} [tr] <-5pt,-5pt> at {+\xrange}  1
	\PLOT "f5-M"
	\put {$\mono$} [tl] <5pt,-5pt> at {-\xrange} 1
	\setdots
	\setlinear
	\plot {-\xrange} -0.35 {+\xrange}  -0.35 /
	\plot {-\xrange} -1.35 {+\xrange}  -1.35 /
	\setsolid
	\putrule from -0.04 -0.35 to +0.04 -0.35
	\put {$+\Lambda^2$} [Bl] <3pt,-3pt> at 0.05 -0.35
	\putrule from -0.04 -1.35 to +0.04 -1.35
	\put {$-\Lambda^2$} [Bl] <3pt,-3pt> at 0.05 -1.35
	\putrule from -0.04 -0.85 to +0.05 -0.85
	\put 0 [Bl] <9pt,-3pt> at 0.05 -0.85
	\put {$U$} [tr] <15pt,-5pt> at {-\xrange} -0.35
	\setcoordinatesystem units <\dimen0,0.5\dimen1> point at 0 1.7
	\setquadratic
	\PLOT "f5-U"
    \endpicture
    \par \bigskip \noindent
    Figure 5:
    \sl Field profiles for the whole Seiberg--Witten domain wall
    ($m=\Lambda/2000$).
    \par
}
$$
\endinput


==> f6.tex <==
%auto-ignore

% Figure 6 for the DomainWall paper
$$
\vbox{
    \hsize=0.8\displaywidth
    \beginpicture
	\setcoordinatesystem units <5.2pc,6pc>
	\setplotarea x from -2.5 to 2.82, y from -0.8 to 1.1
	\arrow <10pt> [0.1,0.3] from -2.5 0 to 2.66 0
	\arrow <10pt> [0.1,0.3] from 0 -.8 to 0 .95 
	\put {$x_3$} [lB] <2pt,2pt> at 2.66 0
	\put {$S^0$} [lB] <2pt,2pt> at 0 .95
	\setquadratic
	\PLOT "f6-S"
	\endpicture
    \hrule height 0pt
    \Tenpoint
    \bigskip\noindent
    Figure~6:
    \sl Qualitative picture of the photino condensate profile
    inside a BPS domain wall.
    \par
    }
$$


==> f7.tex <==
%auto-ignore
%
% Figure 7 for the DomainWall paper
$$
\edef\fvii{\if N\flatsourcedir ./figures/f7/\fi f7.eps}
\vbox{
    \hsize = 0.8\displaywidth
    \centerline{\vbox{%
	\epsfxsize=4cm
	\vbox to 0pt{\hbox to \epsfxsize{\hfil\vrule$\underline{\mskip 2mu U}$}\vss}
	\hrule height 0pt
	\epsfbox{\fvii}
	}}
    \Tenpoint
    \noindent Figure~7:
    {\sl Schematic picture of the winos' stability region  in the complex $U$ plane.}
    The dashed line here represents the marginal stability line~\MarginalStability\
    of the massless SW theory: Winos are stable outside this line but do not exist
    inside it.
    For the SW theory with a small $m\neq0$, the region where
    winos exist is colored white while the region where they are absent from the
    particle spectrum is colored dark grey.
    The two $\bullet$'s indicate the stable vacua $U=\pm\Lambda^2_2$ of the massive
    theory.
    }
$$
\endinput



==> f8.tex <==
%auto-ignore

% Figure 8 for the DomainWall paper
$$
\vbox{
    \hsize=0.8\displaywidth
    \beginpicture
	\setcoordinatesystem units <52pt,2cm>
	\setplotarea x from -3 to 3.4, y from -1 to 1.35
	\arrow <10pt> [0.1,0.3]  from -3 0 to 3.2 0
	\arrow <10pt> [0.1,0.3]  from 0 -1 to 0 1.2
	\put {$x_3$} [Bl] <2pt,2pt> at 3.2 0
	%\setlinear
	%\putrule from -3 0 to 3 0
	%\putrule from 0 -1 to 0 1
	\setquadratic
	\setdots <6pt>
	\setplotsymbol({$\diamond$})
	\PLOT "f8-S1"
	\setplotsymbol({$\circ$})
	\PLOT "f8-S2"
	\setsolid
	\setplotsymbol({.})
	\PLOT "f8-S3"
    \endpicture
    \hrule height 0pt
    \smallskip
    \Tenpoint
    \noindent Figure 8:
    {\sl Qualitative behavior of the gaugino condensates
    in a Seiberg--Witten domain wall.}
    The circles here represent the photino condensate $S^0(x_3)$,
    the diamonds --- the wino condensate $S^\pm(x_3)$ and the
    solid line shows the net gaugino condensate $S(x_3)=S^0+S^\pm$.
    }
$$


==> hyperbasics.tex <==
%auto-ignore
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                         %
% This file is written by Tanmoy Bhattacharya <tanmoy@qcd.lanl.gov> and   %
% is in the public domain for what it is worth. It inserts \specials that %
% are interpreted by (a) the xhdvi hypertex dvi previewer, (b) nextstep   %
% HyperTeXview.app dvi previewer, and (c) the dvipdf driver               %
% For more info, see http://xxx.lanl.gov/hypertex/                        %
%                or  ftp://xxx.lanl.gov/pub/hypertex/index.html           %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                         %
% Only \hyperdef, \hyperref , \href , and \hname are user callable.       %
% Usage: \hyperdef\TeXcs{category}{name}{text}                            %
% Usage: \href{url}{text}                                                 %
% Usage: \hyperref{filename}{category}{name}{text}                        %
%   or   \hyperref\TeXcs{text}                                            %
%             where \TeXcs has been defined by a hyperdef.                %
%                                                                         %
%        Note: The token following \hyperref is expanded completely first.%
%              Really perverse forms like                                 %
%                \csname perverse\endcsname                               %
%              will give an error                                         %
%                                                                         %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The following might be useful to other macros interfacing in.           %
% Usage: \hyper@nchor{name="#myname" href="#refer"}{text}                 %
% Usage: \hyperlink{target_name}{text}                                    %
% Usage: \hypertarget{myname}{text}                                       %
% In cases where there is a possibility of premature expansion use        %
%     \hyper@\hyperpr@ref instead of \hyperref                            %
% and \hyper@\hyperpr@def instead of \hyperdef                            %
% These macros increase enormously in size when expanded, but the expanded%
% token sequence always ends in \hyperpr@ref and \hyperpr@def respectively%
% Macro writers might want to make use of the macro \hyperv@rsion         %
% which is undefined in version 0 and is the version number otherwise     %
% \hyper@nique is exactly like \hyperdef except no special are written    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Save the current catcode of @ and redefine @ to be a letter
%
\expandafter\edef\csname hypers@fe\endcsname{\catcode
                                             `\noexpand @=\the\catcode`\@}%
\catcode`\@=11
%
% Check if the file is already included
%
\ifx\hyperd@ne\hyper@ndefined
 \global\let\hyperd@ne=\relax
\else
 \errhelp{hyperbasics.tex needs to be included only once outside
          of any {...} or \begingroup...\endgroup. You have tried to
          include it more than once. If the previous include was indeed
          outside any groupings, continue and all will be well.}%
 \errmessage{Input this file only once!}%
 \endinput
\fi
%
% Version number
%
\def\hyperv@rsion{8}%
%
% Check and input a previous .hrf file if it exists
%
\newread\hyperf@le
\def\hyperf@lename{\jobname.hrf}%
\immediate\openin\hyperf@le\hyperf@lename\relax
\ifeof\hyperf@le\relax
 \immediate\closein\hyperf@le\relax
\else
 \immediate\closein\hyperf@le\relax
 \input \hyperf@lename
\fi
%
% Open a new .hrf file
%
\newwrite\hyperf@le
\immediate\openout\hyperf@le\hyperf@lename
%%%%
% MAIN SECTION
%%%%
%
% define a token register
%
\newtoks\hypert@ks
%
% Define a convenient macro to hold the character #
%
\edef\hypert@mp{\catcode`\noexpand\#=\the\catcode`\#}%
\catcode`\#=12
\def\hyperh@sh{#}%
\hypert@mp
\let\hypert@mp=\relax
\let\hyper@nd=\relax
\def\hyperstr@pquote"#1"#2\hyper@nd{\ifx\hyper@ndefined#2\hyper@ndefined#1\else
                                    \ifx\hyper@ndefined#1\hyper@ndefined
                                    \hyperstr@pquote#2"\hyper@nd\else
                                    #1\hyperstr@pquote"#2"\hyper@nd\fi\fi}%
\def\hyperstr@pblank" #1 #2\hyper@nd"{\ifx\hyper@ndefined#2\hyper@ndefined#1\else
                                    \ifx\hyper@ndefined#1\hyper@ndefined
                                    \hyperstr@pblank"#2 \hyper@nd"\else
                                    #1\hyperstr@pblank" #2 \hyper@nd"\fi\fi}
%
\long\def\hyper@nchor#1#2{\edef\hyperm@cro{html:<A #1>}%
                          \special\expandafter{\hyperm@cro}%
                          {#2}\special{html:</A>}}%
%
\def\hyper@atm@ning#1->#2\hyper@nd{#2}
\def\hyperlink#1{\edef\hypert@mp{#1}%
               \edef\hypert@mp{\expandafter\hyper@atm@ning\meaning\hypert@mp
                               \hyper@nd}%
               \edef\hypert@mp"{ \expandafter\hyperstr@pquote\expandafter"%
                               \hypert@mp"\hyper@nd}%
               \edef\hypert@mp{\expandafter\hyperstr@pblank\expandafter%
                               "\hypert@mp" \hyper@nd"}%
               \hyper@nchor{href=\expandafter"\hypert@mp"}}%
%
\def\hypertarget#1{\edef\hypert@mp{#1}%
               \edef\hypert@mp{\expandafter\hyper@atm@ning\meaning\hypert@mp
                               \hyper@nd}%
               \edef\hypert@mp"{ \expandafter\hyperstr@pquote\expandafter"%
                               \hypert@mp"\hyper@nd}%
               \edef\hypert@mp{\expandafter\hyperstr@pblank\expandafter%
                               "\hypert@mp" \hyper@nd"}%
               \hyper@nchor{name=\expandafter"\hypert@mp"}}%
%
\def\hyperref{\afterassignment\hyperr@f\let\hyperp@ram}
\def\hyperr@f{\ifx\hyperp@ram{\iffalse}\fi
               \expandafter\expandafter\expandafter\hyperr@@
               \expandafter{%
              \else
               \iffalse}\fi
               \ifx\hyperp@ram\hyper@ndefined
                 \message{Undefined reference}%
                 \def\hyperp@r@m{{}{undefined}{}}%
               \else
                 \edef\hyperp@r@m{\hyperp@ram}%
               \fi
               \expandafter\expandafter\expandafter\hyperr@@
               \expandafter\hyperp@r@m
              \fi}%
% refer to #1, \hyperh@sh#2.#3 or #1\hyperh@sh#2.#3
% depending on what is blank/nonblank
\def\hyperr@@#1#2#3{\ifx\hyper@ndefined#1\hyper@ndefined
                    \hypert@ks\expandafter{\hyperh@sh#2.#3}%
                    \else
                     \ifx\hyper@ndefined#2#3\hyper@ndefined
                      \hypert@ks{#1}%
                     \else
                      \def\hypert@mp{#1}%
                      \hypert@ks\expandafter\expandafter\expandafter
                      {\expandafter\hypert@mp\hyperh@sh#2.#3}%
                     \fi
                    \fi
                    \expandafter\hyperlink\expandafter{\the\hypert@ks}}%
%
% \def\hyperREF#1{\hyperlink{#1}}% % Disabled as per pg's suggestion
%
\def\hyperdef#1#2#3{{\global\escapechar=`\\\relax
                     \edef\hypert@mp{\hyperstr@pquote"#2.#3"\hyper@nd}%
                     \expandafter\ifx\csname hyperd@\meaning\hypert@mp
                     \endcsname
                     \relax
                     \expandafter\gdef\csname hyperd@\meaning\hypert@mp
                     \endcsname{}%
                     \gdef#1{{}{\hyperstr@pquote"#2"\hyper@nd}%
                               {\hyperstr@pquote"#3"\hyper@nd}}%
                     \immediate\write\hyperf@le{\def\noexpand#1{#1}}%
                     \xdef\hypert@mp{\global\let\noexpand\hypert@mp=\relax
                                     \noexpand\hypertarget{\hypert@mp}}%
                     \global\hypert@ks={\hypert@mp}%
                     \else
                     \message\expandafter{'\hypert@mp' duplicate}%
                     \global\let\hypert@mp=\relax
                     \global\hypert@ks={\hyperdef{#1}{#2}{#3@}}%
                     \fi}\the\hypert@ks}%

\def\hyper@nique#1#2#3#4{\global\escapechar=`\\\relax
                     \edef\hypert@mp{\hyperstr@pquote"#2.#3"\hyper@nd}%
                     \expandafter\ifx\csname hyperd@\meaning\hypert@mp
                     \endcsname
                     \relax
                     \gdef#1{{}{\hyperstr@pquote"#2"\hyper@nd}%
                               {\hyperstr@pquote"#3"\hyper@nd}}%
                     \global\let\hypert@mp=\relax
                     #4%
                     \else
                     \global\let\hypert@mp=\relax
                     \hyper@nique{#1}{#2}{#3@}{#4}%
                     \fi
                     }%

%%% 
% protection macros
%%%
\let\hyper@@@@=\relax
\def\hyper@@{\let\hyper@@@=\relax}%
\hyper@@
\def\hyper@{\relax\let\hyper@@@\noexpand\hyper@\noexpand}%
\def\hyperpr@ref{\hyper@@\hyperref}
\def\hyperpr@def{\hyper@@\hyperdef}

% As per pg's suggestion
\let\href\hyperlink
\let\hname\hypertarget
%
% Restore the catcode of @
%
\hypers@fe
\endinput
% A line after endinput to avoid both msdos gremlins and an incomplete
% last line


==> macros.tex <==
%auto-ignore
%&tex
% Macros for the DomainWall paper

\relax\expandafter\ifx\csname TeX\endcsname\relax \input plain \fi
\expandafter\ifx\csname MacroFilesLoaded\endcsname\relax
	\let\next=\relax
    \else
	\wlog{Preloaded macros are not \string\input\space again}%
	\let\next=\endinput
    \fi
    \next
\def\MacroFilesLoaded{YES}

%
% Source directory: Flat or nested
% nested directories require UNIX syntax ./dir/dir/file.tex
%
\ifx\flatsourcedir\UNDEFINED \let\flatsourcedir=Y \fi
\def\include#1#2 {\relax \if Y\flatsourcedir \def\next{\input #2 }%
	\else \def\next{\input #1#2 }\fi \next }
\def\chapterinput{\include{./chapters/}}
%
% load macropackages
%
\expandafter\def\expandafter\JOBNAME\expandafter{\csname\jobname\endcsname}
\def\MACROS{\macros}
\def\FIGSAVER{\figsaver}
\ifx\JOBNAME\MACROS
    \let\terminate=\dump
    \def\dirinput{\include{./}}
\else
    \let\terminate=\endinput
    \let\dirinput=\input
    \ifx\JOBNAME\FIGSAVER \def\dirinput{\include{./../../macros/}}
	\else\def\dirinput{\include{./macros/}}\fi
\fi
\newwrite\phyzzxjunk
\begingroup
	\catcode`\%=12
	\immediate\openout\phyzzxjunk phyzzx.local
	\immediate\write\phyzzxjunk{%auto-ignore}
	\immediate\closeout\phyzzxjunk
	\immediate\openout\phyzzxjunk myphyx.tex
	\immediate\write\phyzzxjunk{%auto-ignore}
	\immediate\closeout\phyzzxjunk
	\endgroup
\let\WLOG=\wlog
\def\wlog#1{}
\dirinput phyzzx
\let\wlog=\WLOG
\dirinput pictex
\dirinput epsf
%
% figure macros
%
\def\figinsert#1{%
    \edef\dirname{\if Y\flatsourcedir\else./figures/#1/\fi}%
    \insert\topins{%
	\penalty 1000 \floatingpenalty 500
	\splittopskip 0pt \splitmaxdepth\maxdimen
	\vbox{\include\dirname #1.tex }\bigskip }}
\def\PLOT "#1"{%
    \immediate\openin\testifexists \dirname #1.saved 
    \ifeof\testifexists
	\immediate\closein\testifexists
	\savelinesandcurves on "\dirname #1.saved"
	\plot "\dirname #1.curve"
	\dontsavelinesandcurves
    \else
	\immediate\closein\testifexists
	\replot "\dirname #1.saved"
    \fi }
%
% Hypertext macros
%
\ifx\makehyperlinks\UNDEFINED \let\makehyperlinks=Y \fi
\if Y\makehyperlinks
    \ifx\hypertarget\UNDEFINED \dirinput hyperbasics.tex \fi
    \begingroup
    \catcode`\@=11
    \gdef\R@FWRITE#1{%
	\ifreferenceopen
	  \else
	    \gl@bal\referenceopentrue
	    \immediate\openout\referencewrite=\jobname.refs
	    \toks@={\begingroup \refoutspecials \catcode`\^^M=10 }%
	    \immediate\write\referencewrite{\the\toks@}%
	  \fi
	\immediate\write\referencewrite{\noexpand\refitem{%
		\noexpand\hypertarget{REF\number\referencecount}%
			{\number\referencecount}}}%
	\p@rse@ndwrite \referencewrite #1%
	}
    \gdef\REFNUM#1{%
	\CheckForOverWrite{#1}\rel@x
	\gl@bal\advance\referencecount by 1
	\xdef#1{\noexpand\hyperlink{REF\number\referencecount}%
			{\number\referencecount}}%
	\csnamech@ck
	\immediate\write\csnamewrite{\def\noexpand#1{\the\referencecount}}%
	}
    \gdef\eqname#1{%
	\gl@bal\advance\equanumber by 1
	\edef\name{CH\number\chapternumber EQ\number\equanumber}%
	\edef\temp{(\chapterlabel.\number\equanumber)}
	\hypertarget{CH\number\chapternumber EQ\number\equanumber}{\temp}%
	\xdef#1{\noexpand\hyperlink{\name}{\noexpand\rm\temp}}%		
	}
    \endgroup
    \else
	\def\href#1#2{#2}
    \fi
%
% Set oneup and two-up formats
%
\ifx\sizeselector\UNDEFINED \let\sizeselector=U \fi %Un-reduced
\newdimen\doublewidth
\doublewidth=72pc
\newinsert\LeftPage
\count\LeftPage=0
\dimen\LeftPage=\maxdimen
\def\PageBox{\vbox{\makeheadline \pagebody \makefootline }}
\def\doubleoutput{%
	\ifvoid\LeftPage \insert\LeftPage{\floatingpenalty 20000 \PageBox}
        \else \shipout\hbox to\doublewidth{\special{landscape}%
            	\box\LeftPage \hfil \PageBox }
	\fi
        \advancepageno
        \ifnum\outputpenalty>-20000 \else \dosupereject \fi
	}
\def\papersize{\hsize=34pc \vsize=50pc \normalspace }
\papersize
\pagebottomfiller=0pt plus 2pt minus 2pt
\skip\footins=20pt plus 8pt minus 6pt
\sectionskip=\bigskipamount
\headskip=\smallskipamount
\everyjob={\relax
    \if R\sizeselector
	\mag=833
	\voffset=-0.45truein
	\hoffset=-0.45truein
	\output={\doubleoutput}
	\message{Warning: some DVI drivers cannot handle reduced output!!!}
    \else
	\mag=1000
	\voffset=0pt
	\hoffset=0pt
    \fi
    }
\the\everyjob
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\NS{{\cal N}}
\def\SS{{\cal S}}
\def\N {{N_c}}
\def\mono{{\cal M}}
\def\amono{\widetilde{\mono}}
\def\dyon{{\cal D}}
\def\adyon{\widetilde{\dyon}}
\let\modulo=\mod
\def\mod{T}
\let\Imaginary=\Im
\let\Real=\Re
\def\Im{\mathop{\rm Im}\nolimits}
\def\Re{\mathop{\rm Re}\nolimits}
%\def\Vnote{\footnote{\bf VK}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begingroup
\catcode`\@=11
\gdef\journal#1&#2(#3){\begingroup \let\journal=\dummyj@urnal
    \unskip, \sl #1\unskip~\bf\ignorespaces #2\rm
    (\afterassignment\j@ur \count255=#3) \endgroup\ignorespaces }
\gdef\jjournal#1&#2(#3){\begingroup \let\journal=\dummyj@urnal
    \sl #1\unskip~\bf\ignorespaces #2\rm
    (\afterassignment\j@ur \count255=#3) \endgroup\ignorespaces }
\endgroup
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\terminate

